Correctly Communicating Software: Distributed, Asynchronous, and Beyond (extended version)

Much of the software we use in everyday life consists of distributed components (running on separate cores or even computers) that collaborate through communication (by exchanging messages). It is crucial to develop robust methods that can give reliable guarantees about the behavior of such message-passing software. With a focus on session types as communication protocols and their foundations in logic, this thesis revolves around the following question: How can we push the boundaries of the logical foundations of session types (binary and multiparty), extending their expressiveness and applicability, while preserving fundamental correctness properties? In this context, this thesis studies several intertwined aspects of message-passing.

==> repos/pi-bi/paper/calculus.tex <==
% !TeX root = ../../../main.tex
\section{The \piBI Calculus}
\label{sec:pibi}

%<*piBI:piBI>
In this section we formally introduce \piBI, a \picalc with constructs for session-based concurrency~\cite{conf/concur/Honda93,conf/esop/HondaVK98} and our new spawn prefix.
We first describe syntax and dynamics (reduction semantics), and then present its associated type system, based on the sequent calculus for \BI.
Following \piDILL~\cite{conf/concur/CairesP10,journal/mscs/CairesPT16}, our type system for \piBI admits a ``provide/use'' reading for typable processes, whereby a specific channel \emph{provides} a session by \emph{using} zero or more other sessions.

%<*alphalamda:piBI>
\paragraph{Notation.}

We assume an enumerable set of \emph{names} $a,b,c,\ldots,x,y,z \in \Name$ to denote channels.
We make use of finite partial functions~$f \from A \fpfn B$.
We write~$f(x) = \bot$ if~$f$ is not defined on~$x$.
We define~$\dom(f) = \{ x \in A \mid f(x) \neq \bot \}$.
We write $ \map{a_1 -> b_1; \dots ;a_n -> b_n} $ to denote a map,
and~$\emptymap$ for the empty map.
We will also use set comprehensions for finite functions,
e.g., $\map{a -> b | a \in \{1,2\}, b = a^2}$.
For a finite partial function~$f$ and a set~$X$, we write~$f \setminus X$ for the function that coincides with~$f$ except for being undefined on~$X$.
We write $\Pow(A)$ to denote the powerset of set $A$.
%</alphalamda:piBI>
%</piBI:piBI>

\subsection{Process Syntax}
\label{sec:procs}

%<*piBI:piBI:syntax>
%<*alphalamda:piBI:syntax>
\begin{figure}[t]
    \begin{align*}
        P,Q,R &
        \begin{array}[t]{@{}l@{}lr@{\kern2em}l@{\kern1em}lr@{}}
            {} ::= {} &
            \pOut* x[y] ; ( P \| Q ) & \text{send}
            & \sepr &
            \pIn x(y) ; P & \text{receive}
            \\ \sepr* &
            \pClose x[] & \text{close}
            & \sepr &
            \pWait x() ; P & \text{wait}
            \\ \sepr* &
            \pSelL x ; P & \text{left selection}
            & \sepr &
            \pBraLR x > {P}{Q} & \text{branch}
            \\ \sepr* &
            \pSelR x ; P & \text{right selection}
            & \sepr &
            \pFwd [x<>y] & \text{forwarder}
            \\ \sepr* &
            \pRes{x} ( P \| Q ) & \text{restriction + parallel}
            & \sepr &
            \pSpw[\spvar] ; P & \text{spawn}
        \end{array}
    \end{align*}

    \caption{Syntax of \piBI processes.}
    \ifalphalambda \label{f:alphalambda:piBI:processes}
    \else \label{f:piBI:processes} \fi
\end{figure}

The syntax of \piBI processes is given in \ifalphalambda\Cref{f:alphalambda:piBI:processes}\else\Cref{f:piBI:processes}\fi.
The structure and conventions of process calculi based on Curry-Howard correspondences are typically based on implicit expectations of how the components of a system are organized---an expectation that is ultimately verified by typing.
The idea is that interaction is grouped into a \emph{session}, the sequence of interactions along a single channel.
As hinted at above, a process~$P$ should \emph{provide} a session at some specific channel~$x \in \fn(P)$, and there is always a single \emph{user} of the session exchanging messages with~$P$ along~$x$.
To provide a session, a process can make use of sessions on other channels.
\ifthesis\else

\fi
\ifthesis\else\ifappendix\else\pagebreak\fi\fi
Most constructs are standard and reflect these expectations:
\begin{itemize}
    \item
        \emph{Receive/Send:}
        A process $\pIn x(y) ; P$ receives a channel~$y$ from the session at~$x$ and proceeds as~$P$, continuing the session at~$x$.

        A process $\pOut* x[y] ; \big( P \| Q \big)$ sends a \emph{fresh} channel~$y$ over the session at~$x$; the process~$P$ provides the new session at~$y$, while~$Q$ continues the session at~$x$.

    \item
        \emph{Labeled choice (selection and branching):}
        The processes $\pSelL x ; P$ and $\pSelR x ; P$ select left/right labels over the session at~$x$, respectively.
        The dual process $\pBraLR x > {P}{Q}$ offers these left/right options, which trigger continuation~$P$ or~$Q$, respectively.

    \item
        \emph{Explicit session closing:}
        The end of a session is expected to be explicitly closed by a final handshake between the dual prefixes $\pClose x[]$ and $\pWait x() ; P$ (empty send/receive, respectively).

    \item
        \emph{Structured parallel composition:}
        Parallel composition\ifalphalambda \else, in keeping with \piDILL~\cite{journal/mscs/CairesPT16},\fi is used jointly with restriction.
        In a process~$\pRes{x} ( P \| Q )$ a new session is created at~$x$, provided by~$P$ with~$Q$ as its only user.
        To improve readability, we sometimes annotate the parallel operator with the name of the associated restriction, and write $\pRes{x} ( P \|_x Q )$.

    \item
        \emph{Forwarders:}
        A process $\pFwd [x<>y]$ provides a session at~$x$ as a copycat of the session at~$y$.
\end{itemize}

The key novel construct of \piBI is the \emph{spawn prefix} $\pSpw[\spvar] ; P$.
It is parametrized by what we call a \emph{spawn binding}~$\spvar$.
Spawn bindings, formally defined below, are a unification and generalization of prefixes like $\pSpw[x->x_1,x_2]$ (copy the session at $x$ to $x_1$ and $x_2$) but also $\pSpw[x->\emptyset]$ (drop the session at $x$).
Indeed, in addition to allowing the simultaneous mapping of more than one name~$x$, we allow names to be mapped to sets of names, encompassing the nullary and binary cases above.

\begin{definition}[Spawn Binding]
    \ifalphalambda \label{d:alphalambda:spawnEnv}
    \else \label{d:piBI:spawnEnv} \fi
    A finite partial function ${\spvar \from \Name \fpfn \Pow(\Name)}$ is a \emph{spawn binding}~if:
    \begin{itemize}
        \item
            $\forall x,y \in \dom(\spvar).~ x \neq y \implies \spvar(x) \cap \spvar(y) = \emptyset$, and
        \item
            $\forall x \in \dom(\spvar) .~ \dom(\spvar) \cap \spvar(x) = \emptyset$.
      \end{itemize}

      We define the \emph{restrictions} of~$\spvar$ to be the set $\restrOf(\spvar) = \bigcup_{x \in \dom(\spvar)} \spvar(x)$.
      We omit redundant delimiters in spawn prefixes, e.g., we write $\pSpw[x->x_1,x_2; y->y_1]$ for $\pSpw[\map{x->\{x_1,x_2\}; y->\{y_1\}}]$.

      Given two spawn bindings~$\spvar_1$ and~$\spvar_2$ we say they are \emph{independent}, written~${\spvar_1 \indep \spvar_2}$, if
      $\dom(\spvar_1) \cap \dom(\spvar_2) = \emptyset$,
      $\dom(\spvar_1) \cap \restrOf(\spvar_2) = \emptyset$,
      $\restrOf(\spvar_1) \cap \restrOf(\spvar_2) = \emptyset$, and
      $\dom(\spvar_2) \cap \restrOf(\spvar_1) = \emptyset$.
\end{definition}

\paragraph{Free and bound names.}

Except for the new spawn construct, the notion of free and bound names is standard: the processes $\pOut* x[y] ; ( P \| Q )$, $\pIn x(y) ; P$, and $\pRes{y} ; ( P \| Q )$ all bind~$y$.
For the spawn prefix, the situation is a bit different.
Given a set of names $X$, a spawn~$\pSpw[x->X] ; P$ signals to the context that $P$ will use $n=|X|$ times the session at~$x$.
The names in~$X$ indicate the new names that $P$ will use instead of~$x$.
As such, these new names are bound in~$P$ by the spawn prefix, whereas the original name $x$ is free in~$P$.
Formally, $\fn(\pSpw[\spvar] ; P) = \big( \fn(P) \setminus \restrOf(\spvar) \big) \cup \dom(\spvar)$.

We implicitly identify processes up to $\alpha$-conversion and we adopt Barendregt's variable convention: all bound names are different, and bound names are different from free names.

\paragraph{Structural congruence.}

\begin{figure}[t]
    \ifthesis
    \begin{mathpar}
        \begin{bussproof}[cong-assoc-L]
            \bussAssume{
                x \notin \fn(Q)
            }
            \bussAssume{
                y \notin \fn(P)
            }
            \bussBin{
                \pRes{x} \big( P \|_x \pRes{y} ( Q  \|_y R ) \big)
                \congr
                \pRes{y} \big( Q \|_y \pRes{x} ( P  \|_x R ) \big)
            }
        \end{bussproof}
        \and
        \begin{bussproof}[cong-assoc-R]
            \bussAssume{
                x \notin \fn(R)
            }
            \bussAssume{
                y \notin \fn(P)
            }
            \bussBin{
                \pRes{x} \big( P \|_x \pRes{y} ( Q  \|_y R ) \big)
                \congr
                \pRes{y} \big( \pRes{x} ( P  \|_x Q ) \|_y R \big)
            }
        \end{bussproof}
        \and
        \begin{bussproof}[cong-spawn-swap]
            \bussAssume{
                \spvar_1 \indep \spvar_2
            }
            \bussUn{
                \pSpw[\spvar_1] ; \pSpw[\spvar_2] ; Q
                \equiv
                \pSpw[\spvar_2] ; \pSpw[\spvar_1] ; Q
            }
        \end{bussproof}
    \end{mathpar}
    \else
    \input{figures/congr.tex}
    \fi

    \caption{Structural congruence.}
    \ifalphalambda \label{f:alphalambda:piBI:cong}
    \else \label{f:piBI:cong} \fi
\end{figure}

As usual, we define a congruence that identifies processes up to inconsequential syntactical differences.
\emph{Structural congruence}, denoted $\congr$, is the smallest congruence satisfying the rules in \ifalphalambda\Cref{f:alphalambda:piBI:cong}\else\Cref{f:piBI:cong}\fi:
the orders of parallel compositions and independent spawn prefixes do not matter (\ifthesis{}Rules~\ruleLabel{cong-assoc-R}, \ruleLabel{cong-assoc-L}, and~\ruleLabel{cong-spawn-swap}\else\cref{cong-assoc-r,cong-assoc-l} and \cref{cong-spawn-swap}\fi, respectively).
%</alphalamda:piBI:syntax>

Our structural congruence is a bit more fine-grained than is usual for the \picalc.
This is guided by the desire to make typing consistent under structural congruence.
Typing will enforce the expectations of process structure alluded to before, so our congruence needs to preserve them.
For example, in a process $\pOut* x[y] ; ( P \| Q )$ we expect $P$ to provide the new session at~$y$ and~$Q$ to continue the session at~$x$.
Admitting commutativity of parallel would break this expectation.
Similarly, in the composition of processes $\pRes{x} ( P \| Q )$ it is important that $P$ provides the session that governs $x$, and that $Q$ dually uses the session at $x$.
This choice of structural congruence simplifies the technical development and makes the correspondence between logic and type theory sharper.
%</piBI:piBI:syntax>

\subsection{Reduction Semantics}
\label{sec:red-sem}

%<*piBI:piBI:reduction>
%<*alphalamda:piBI:semantics>
The operational semantics of \piBI is defined in terms of a reduction relation, denoted~$\redd$, which combines the usual reductions of the \picalc with reductions
for spawn prefixes.
As usual, we shall write $\redd*$ to denote the reflexive, transitive closure of $\redd$, and $P \nredd$ when $P$ cannot reduce.

\begin{figure}[t]
    \begin{mathpar}
        \begin{bussproof}[red-recv-send]
            \bussAx{
                \pRes{x} \big( \pIn x(y) ; Q \|_x \pOut* x[y] ; ( P_1 \| P_2 ) \big)
                \redd
                \pRes{x} \big( \pRes{y} ( P_1 \|_y Q ) \|_x P_2 \big)
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-wait-close]
            \bussAx{
                \pRes{x} \big( \pWait x() ; Q \|_x \pClose x[] \big)
                \redd
                Q
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-send-recv]
            \bussAx{
                \pRes{x} \big( \pOut* x[y] ; ( P_1 \| P_2 ) \|_x \pIn x(y) ; Q \big)
                \redd
                \pRes{x} \big( P_2 \|_x \pRes{y} ( P_1 \|_y Q ) \big)
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-close-wait]
            \bussAx{
                \pRes{x} \big( \pClose x[] \|_x \pWait x() ; Q \big)
                \redd
                Q
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-sel-bra]
            \bussAssume{
                \ell \in \{ \inl , \inr \}
            }
            \bussUn{
                \pRes{x} \big( \pSel* x < \ell ; P \|_x \pBraLR x > {Q_{\inl}}{Q_{\inr}} \big)
                \redd
                \pRes{x} \big( P \|_x Q_\ell \big)
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-fwd-R]
            \bussAx{
                \pRes{x} ( P \|_x \pFwd [y<>x] )
                \redd
                P \{ y/x \}
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-fwd-L]
            \bussAx{
                \pRes{x} ( \pFwd [x<>y] \|_x P )
                \redd
                P \{ y/x \}
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-spawn]
            \bussAssume{
                \spvar(x) = \{x_1,\ldots,x_n\}
            }
            \bussAssume{
                \spvar' = \big( (\spvar \setminus \{x\}) \cup \map{ z -> \{z_1,\ldots,z_n\} | z \in \fn(P) \setminus \{x\} } \big)
            }
            \bussBin{
                \pRes{x} ( P \|_x \pSpw[\spvar] ; Q )
                \redd
                \pSpw[\spvar'] ; \pRes{x_1} \big( \idx{P}{1} \|_{x_1} \ldots \pRes{x_n} ( \idx{P}{n} \|_{x_n} Q ) \ldots \big)
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-spawn-R]
            \bussAssume{
                x \notin \dom(\spvar)
            }
            \bussUn{
                \pRes{x} ( P \|_x \pSpw[\spvar] ; Q )
                \redd
                \pSpw[\spvar] ; \pRes{x} ( P \|_x Q )
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-spawn-L]
            \bussAssume{
                x \notin \dom(\spvar)
            }
            \bussUn{
                \pRes{x} ( \pSpw[\spvar] ; P \|_x Q )
                \redd
                \pSpw[\spvar] ; \pRes{x} ( P \|_x Q )
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-spawn-merge]
            \bussAx{
                \pSpw[\spvar_1] ; \pSpw[\spvar_2] ; P
                \redd
                \pSpw[\spvar_1 \spmerge \spvar_2] ; P
            }
        \end{bussproof}
        \\
        \evalCtx{K}
        \begin{array}[t]{@{}l@{}l@{}}
            {} ::= {} &
            \evalHole
            \sepr
            \pSpw[\spvar] ; \evalCtx{K}
            \\ \sepr* &
            \pRes{x} ( P \|_x \evalCtx{K} )
            \\ \sepr* &
            \pRes{x} ( \evalCtx{K} \|_x P )
        \end{array}
        \and
        \begin{bussproof}[red-eval-ctx](t)
            \bussAssume{
                P
                \redd
                Q
            }
            \bussUn{
                \evalCtx{K}[P]
                \redd
                \evalCtx{K}[Q]
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-cong](t)
            \bussAssume{
                P \congr P'
            }
            \bussAssume{
                P'
                \redd
                Q'
            }
            \bussAssume{
                Q' \congr Q
            }
            \bussTern{
                P
                \redd
                Q
            }
        \end{bussproof}
    \end{mathpar}

    \caption{Reduction rules for \piBI.}
    \ifalphalambda \label{f:alphalambda:piBI:reduction}
    \else \label{f:piBI:reduction} \fi
\end{figure}

\ifalphalambda\Cref{f:alphalambda:piBI:reduction} \else\Cref{f:piBI:reduction} \fi gives the reduction rules.
The first seven rules describe interactions along a channel.
Rules~\ruleLabel{red-recv-send} and~\ruleLabel{red-send-recv} describe the exchange of channel~$y$ along~$x$.
The resulting process contains an explicit restriction for~$y$ with $P_2$ out of scope, reflecting the expectation that~$P_1$ is the provider of the new session at~$y$.
Rules~\ruleLabel{red-wait-close} and~\ruleLabel{red-close-wait} describe the closing of a session at~$x$.
Rule~\ruleLabel{red-sel-bra} shows how a branch offered on~$x$ can be selected by sending $\inl$ or $\inr$.
Finally, Rules~\ruleLabel{red-fwd-R} and~\ruleLabel{red-fwd-L} explain the elimination of a forwarder connected by restriction in terms of a substitution.

The next four rules of \ifalphalambda \Cref{f:alphalambda:piBI:reduction} \else \Cref{f:piBI:reduction} \fi define the semantics of spawn.
The crucial rule is Rule~\ruleLabel{red-spawn}, which \ifalphalambda\else we explain by example.

\newpage
\begin{example}
    \label{x:piBI:contraction}
    Consider a process $P$ that provides a session on channel $x$.
    Another process~$Q$ provides a session on $v$ by relying \emph{twice} on the session provided by $P$, on channels $x_1$ and~$x_2$.
    Concrete examples are $P \deq \pClose x[]$ and $Q \deq \pWait x_1() ; \pWait x_2() ; \pClose v[]$.
    Now consider the following process:
    \[
        R \deq \pRes{x} \big( \pWait z() ; P \|_x \pSpw[x->x_1,x_2] ; Q \big)
    \]
    In $R$, the process $P$ is blocked waiting for the session on~$z$ to close.
    By Rule~\ruleLabel{red-spawn},
    \[
        R \redd \pSpw[z->z_1,z_2] ; \pRes{x_1} \big( \pWait z_1() ; P \{ x_1/x \} \|_{x_1} \pRes{x_2} ( \pWait z_2() ; P \{ x_1/x \} \|_{x_2} Q ) \big).
    \]
    The result is two copies of $P$, providing their sessions on $x_1$ and $x_2$ instead of on $x$.
    Since we are also copying the closing prefixes on $z$, an additional spawn is generated, but now on $z$: it signals to the environment that two copies of the process providing the session on $z$ should be created and that they should provide its session on $z_1$ and $z_2$.
\end{example}

In the example above, the channel $z$ is a free name of the process that is copied by the spawn reduction.
Generally, a copied process may rely on arbitrarily many sessions on the free names of the process, and all the processes providing these sessions will have to be copied as well.
To handle the general case, Rule~\ruleLabel{red-spawn} \fi uses the following definition.

\begin{definition}[Indexed Renaming]
    \ifalphalambda \label{d:alphalambda:idxRenaming}
    \else \label{d:piBI:idxRenaming} \fi
    Given a process~$P$ with $\fn(P) = \{a,b,\dots,z\}$, we define~$\idx{P}{i}$ to be the process~$P$ where every free name is replaced by a fresh copy of the name indexed by~$i$.
    Formally, assuming $a_i,b_i,\dots,z_i \notin \fn(P)$, $\idx{P}{i} \deq P \{ a_i/a,b_i/b,\ldots,z_1/z \}$.
\end{definition}

\ifalphalambda
Rule~\ruleLabel{red-spawn} then duplicates or discards a process as specified by the involved spawn binding (\Cref{d:alphalambda:spawnEnv}), propagating the spawn accordingly.
\else
Note that Rule~\ruleLabel{red-spawn} uniformly handles the case where a session is not used at all.

\begin{example}
    \label{x:piBI:weakening}
    Consider again $P$ from \Cref{x:piBI:contraction} that provides a session on $x$.
    This time, the process $Q'$ (adapted from \Cref{x:piBI:contraction}) provides a session on $v$ \emph{without} relying on the session provided by $P$ (i.e., simply $Q' \deq \pClose v[]$).
    Now consider the following process, obtained by replacing the spawn prefix and $Q$ in $R$ from \Cref{x:piBI:contraction}:
    \[
        R' \deq \pRes{x} \big( \pWait z() ; P \|_x \pSpw[x->\emptyset] ; Q' \big)
    \]
    By Rule~\ruleLabel{red-spawn}, $R' \redd \pSpw[z->\emptyset] ; Q'$.
    In this case, $P$ is dropped.
    Since the empty receive on $z$ is also dropped, an additional spawn is generated to signal to the environment that the process providing the session on $z$ should be dropped as well.
\end{example}
\fi

Rules~\ruleLabel{red-spawn-R}, \ruleLabel{red-spawn-L}, and~\ruleLabel{red-spawn-merge} show how the spawn prefix interacts with independent process compositions and with other spawn prefixes, respectively.
Rules~\ruleLabel{red-spawn-R} and~\ruleLabel{red-spawn-L} are forms of scope extrusion: spawn prefixes can ``bubble up'' past restrictions that do not capture their bindings, possibly enabling interactions of the spawn with processes in the outer context.
Rule~\ruleLabel{red-spawn-merge} describes how two consecutive spawn prefixes
can be combined into a single spawn, by merging the spawn bindings, denoted $\spmerge$, as follows.

\begin{definition}[Merge]
    \ifalphalambda \label{d:alphalambda:merge}
    \else \label{d:piBI:merge} \fi
    Let $\spvar[X] \deq \bigcup \{ \spvar(x) \mid x \in X \cap \dom(\spvar) \}.$
    The \emph{merge} of two spawn bindings~$\spvar_1, \spvar_2$,
    written $\spvar_1 \spmerge \spvar_2$, is defined as:
    \[
        (\spvar_1 \spmerge \spvar_2)(x) \deq \begin{cases}
            \spvar_2[\spvar_1(x)] \cup (\spvar_1(x) \setminus \dom(\spvar_2))
            & \text{if $x \in \dom(\spvar_1)$}
            \\
            \spvar_2(x)
            & \text{if $x \notin \dom(\spvar_1) \cup \restrOf(\spvar_1)$}
            \\
            \bot
            & \text{otherwise}
        \end{cases}
    \]
\end{definition}

\ifalphalambda\else
\noindent
Note that the merge of two independent spawn bindings is just disjoint union (as functions), and $\emptyset$ is the neutral element for $\spmerge$.
Merge is associative:
$(\spvar_1 \spmerge (\spvar_2 \spmerge \spvar_3)) = ((\spvar_1 \spmerge \spvar_2) \spmerge \spvar_3)$.

\begin{figure}[t]
    \begin{center}
        \ifthesis
        \input{\dirOOPSLA/figures/merge_ex.tikz}
        \else
        \input{figures/merge_ex.tikz}
        \fi
    \end{center}
    \caption{Graphical illustration of merge (\Cref{d:piBI:merge}).}\label{f:piBI:merge}
\end{figure}

The idea behind the merge operation $\spvar_1 \spmerge \spvar_2$ is to ``connect'' the outputs of~$\spvar_1$ to the inputs of~$\spvar_2$, similarly to composition of relations.
However, names that are irrelevant for~$\spvar_1$ should still be subject to the mapping of~$\spvar_2$, unless they are captured by the restrictions of~$\spvar_1$.
For example:
\[
    \map*{
        \begin{matrix*}[l]
            x -> \emptyset,
            \\
            y -> \{y_1, y_2, y_3\}
        \end{matrix*}
    }
    \spmerge
    \map*{
        \begin{matrix*}[l]
            y_2 -> \emptyset,
            \\
            y_3 -> \{y_4, y_5\},
            \\
            z -> z_1
        \end{matrix*}
    }
    =
    \map*{
        \begin{matrix*}[l]
            x -> \emptyset,
            \\
            y -> \{y_1, y_4, y_5\},
            \\
            z -> z_1
        \end{matrix*}
    }
\]
\Cref{f:piBI:merge} graphically illustrates this.
Note how~$x$ and~$z$ are both in the domain of the result,
and how the mapping to~$y_1$ is preserved by the merge,
although it is not in the restrictions of the second binding.
\fi

The last two rules in \ifalphalambda \Cref{f:alphalambda:piBI:reduction} \else \Cref{f:piBI:reduction} \fi are purely structural.
Rule~\ruleLabel{red-eval-ctx} closes reduction under \emph{evaluation contexts}, denoted~$\evalCtx{K}$, consisting of spawn prefixes and structured parallel compositions (cf.\ \ifalphalambda \Cref{f:alphalambda:piBI:reduction} \else \Cref{f:piBI:reduction} \fi for its definition).
Rule~\ruleLabel{red-cong} closes reduction under structural congruence.
%</piBI:piBI:reduction>
%</alphalamda:piBI:semantics>

\subsection{Typing}
\label{sec:typing}

%<*piBI:piBI:typing>
%<*alphalamda:piBI:typing>
The \piBI type system is based on the \BI sequent calculus, and follows the approach of \piDILL: propositions are interpreted as session types, where the context governs the \emph{use} of available channels and the conclusion governs the process' behavior on the \emph{provided} channel.
As such, the type system of \piBI uses judgments of the form $\Delta \vdash P \typInf x:A$, where the process $P$ provides the session $A$ on channel $x$, while using the sessions provided by the typing context $\Delta$.

\begin{figure}[p]
    \def\MathparLineskip{\lineskip=3pt}
    \def\defaultHypSeparation{\hskip1ex}
    \ifalphalambda\else
    %<*alphalambda:alphalambda:types>
    Types, bunches, and contexts:
    \vspace{-1.5ex}
    \begin{align*}
        & \begin{array}[t]{@{}r@{}l@{}lr@{}}
            A,B,C
            & {} ::= {} &
            \mOne
            \sepr*
            A \sep B
            \sepr*
            A \wand B
            & \text{multiplicatives}
            \\ & \sepr* &
            \aOne
            \sepr*
            A \land B
            \sepr*
            A \to B
            \sepr*
            A \lor B
            & \text{additives}
            \\
            \Delta, \Theta
            & {} ::= {} &
            \mEmpty
            \sepr*
            \aEmpty
            \sepr*
            x:A
            \sepr*
            \Delta , \Delta
            \sepr*
            \Delta ; \Delta
            & \text{bunches}
            \\
            \bunchCtx{\Gamma}
            & {} ::= {} &
            \bunchHole
            \sepr*
            \Delta , \bunchCtx{\Gamma}
            \sepr*
            \Delta ; \bunchCtx{\Gamma}
            \sepr*
            \bunchCtx{\Gamma} , \Delta
            \sepr*
            \bunchCtx{\Gamma} ; \Delta
            & \text{bunched contexts}
        \end{array}
    \end{align*}
    %</alphalambda:alphalambda:types>

    \dashes

    Typing:
    \vspace{-1.5ex}
    \fi
    \begin{mathpar}
        \begin{bussproof}[typ-sep-R]
            \bussAssume{
                \Delta_1 \vdash P_1 \typInf y:A
            }
            \bussAssume{
                \Delta_2 \vdash P_2 \typInf x:B
            }
            \bussBin{
                \Delta_1 , \Delta_2 \vdash \pOut* x[y] ; ( P_1 \| P_2 ) \typInf x:A \sep B
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-sep-L]
            \bussAssume{
                \bunchCtx{\Gamma}[x:B , y:A] \vdash P \typInf z:C
            }
            \bussUn{
                \bunchCtx{\Gamma}[x:A \sep B] \vdash \pIn x(y) ; P \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-wand-R]
            \bussAssume{
                \Delta , y:A \vdash P \typInf x:B
            }
            \bussUn{
                \Delta \vdash \pIn x(y) ; P \typInf x:A \wand B
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-wand-L]
            \bussAssume{
                \Delta \vdash P_1 \typInf y:A
            }
            \bussAssume{
                \bunchCtx{\Gamma}[x:B] \vdash P_2 \typInf z:C
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta , x:A \wand B] \vdash \pOut* x[y] ; ( P_1 \| P_2 ) \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-emp-R]
            \bussAx{
                \mEmpty \vdash \pClose x[] \typInf x:\mOne
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-emp-L]
            \bussAssume{
                \bunchCtx{\Gamma}[\mEmpty] \vdash P \typInf z:C
            }
            \bussUn{
                \bunchCtx{\Gamma}[x:\mOne] \vdash \pWait x() ; P \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-conj-R]
            \bussAssume{
                \Delta_1 \vdash P_1 \typInf y:A
            }
            \bussAssume{
                \Delta_2 \vdash P_2 \typInf x:B
            }
            \bussBin{
                \Delta_1 ; \Delta_2 \vdash \pOut* x[y] ; ( P_1 \| P_2 ) \typInf x:A \land B
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-conj-L]
            \bussAssume{
                \bunchCtx{\Gamma}[x:B ; y:A] \vdash P \typInf z:C
            }
            \bussUn{
                \bunchCtx{\Gamma}[x:A \land B] \vdash \pIn x(y) ; P \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-impl-R]
            \bussAssume{
                \Delta ; y:A \vdash P \typInf x:B
            }
            \bussUn{
                \Delta \vdash \pIn x(y) ; P \typInf x:A \to B
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-impl-L]
            \bussAssume{
                \Delta \vdash P_1 \typInf y:A
            }
            \bussAssume{
                \bunchCtx{\Gamma}[x:B] \vdash P_2 \typInf z:C
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta ; x:A \to B] \vdash \pOut* x[y] ; ( P_1 \| P_2 ) \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-true-R]
            \bussAx{
                \aEmpty \vdash \pClose x[] \typInf x:\aOne
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-true-L]
            \bussAssume{
                \bunchCtx{\Gamma}[\aEmpty] \vdash P \typInf z:C
            }
            \bussUn{
                \bunchCtx{\Gamma}[x:\aOne] \vdash \pWait x() ; P \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-disj-R-inl]
            \bussAssume{
                \Delta \vdash P \typInf x:A
            }
            \bussUn{
                \Delta \vdash \pSelL x ; P \typInf x:A \lor B
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-disj-L-inl]
            \bussAssume{
                \Delta \vdash P \typInf x:B
            }
            \bussUn{
                \Delta \vdash \pSelR x ; P \typInf x:A \lor B
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-fwd]
            \bussAx{
                y:A \vdash \pFwd [x<>y] \typInf x:A
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-cut]
            \bussAssume{
                \Delta \vdash P \typInf x:A
            }
            \bussAssume{
                \bunchCtx{\Gamma}[x:A] \vdash Q \typInf x:C
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta] \vdash \pRes{x} ( P \| Q ) \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-struct]
            \bussAssume{
                \Delta_2 \vdash P \typInf z:C
            }
            \bussAssume{
                \spvar : \Delta_1 \tobunch \Delta_2
            }
            \bussBin{
                \Delta_1 \vdash \pSpw[\spvar] ; P \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-bunch-equiv]
            \bussAssume{
                \Delta_2 \vdash P \typInf z:C
            }
            \bussAssume{
                \Delta_2 \equiv \Delta_1
            }
            \bussBin{
                \Delta_1 \vdash P \typInf z:C
            }
        \end{bussproof}
    \end{mathpar}

    \dashes

    Spawn binding:
    \vspace{-1.5ex}
    \begin{mathpar}
        \begin{bussproof}[spawn-contract]
            \bussAx{
                \map{x -> \{x_1,\ldots,x_n\} | x \in \Delta}
                :
                \bunchCtx{\Gamma}[\Delta] \tobunch \bunchCtx{\Gamma}[\idx{\Delta}{1} ; \ldots ; \idx{\Delta}{n}]
            }
        \end{bussproof}
        \and
        \begin{bussproof}[spawn-weaken]
            \bussAx{
                \map{x -> \emptyset | x \in \Delta_1}
                :
                \bunchCtx{\Gamma}[\Delta_1 ; \Delta_2] \tobunch \bunchCtx{\Gamma}[\Delta_2]
            }
        \end{bussproof}
        \and
        \begin{bussproof}[spawn-merge]
            \bussAssume{
                \spvar_1 : \Delta_1 \tobunch \Delta_2
            }
            \bussAssume{
                \spvar_2 : \Delta_2 \tobunch \Delta_3
            }
            \bussBin{
                (\spvar_1 \spmerge \spvar_2) : \Delta_1 \tobunch \Delta_3
            }
        \end{bussproof}
    \end{mathpar}

    \caption{\ifalphalambda{}T\else{}Types, t\fi{}yping rules and spawn binding rules for \piBI.}
    \ifalphalambda \label{f:alphalambda:piBI:typing}
    \else \label{f:piBI:typing} \fi
\end{figure}

\ifalphalambda
The top of \Cref{f:alphalambda:piBI:typing} gives types, bunches, and bunched contexts; we explain the session behavior associated with types when we discuss the typing rules below.
%<*alphalambda:alphalambda:bunch>
Bunches~$\Delta$ are binary trees with internal nodes labelled with either `$\,;\,$' or `$\,,\,$', and with leaves being either unit bunches ($\mEmpty$ or $\aEmpty$) or typing assignments ($x : A$).
We write~\ifalphalambda$\fv(\Delta)$\else$\fn(\Delta)$\fi for the set of \ifalphalambda variables \else names \fi occurring in the bunch~$\Delta$, and write $x \in \Delta$ to denote \ifalphalambda$x \in \fv(\Delta)$\else$x \in \fn(\Delta)$\fi.
\ifalphalambda\else
%<*alphalambda:alphalambda:bunchEquiv>
\ifalphalambda\else As is standard for \BI, we consider bunches modulo \fi the least congruence on bunches closed under commutative monoid laws for `$\,,\,$' with unit $\mEmpty$, and for `$\,;\,$' with unit $\aEmpty$, denoted~$\equiv$.
For example, $(\Delta_1 , \mEmpty) ; \Delta_2 \equiv \Delta_2 ; \Delta_1$.
%</alphalambda:alphalambda:bunchEquiv>
\fi

Bunched contexts $\bunchCtx{\Gamma}$ are bunches with a hole $\bunchHole$.
As usual, we write $\bunchCtx{\Gamma}[\Delta]$ for a bunch obtained by replacing $\bunchHole$ with $\Delta$ in $\bunchCtx{\Gamma}$.
We write $\bunchCtx{\Gamma}[\bunchHole \mid \ldots \mid \bunchHole]$ for a bunched context with multiple holes.
%</alphalambda:alphalambda:bunch>
\fi

\ifalphalambda
Types, bunches, and bunched context are the same for \piBI as for the \alcalc given in \Cref{f:alphalambda:typing}.
\fi
\ifalphalambda\Cref{f:alphalambda:piBI:typing} \else\Cref{f:piBI:typing} also \fi gives the type system for \piBI.
We organize them in four groups:
the first six rules type communication primitives with multiplicative types, and the next six rules with additive types;
the following three rules type branching primitives using disjunction;
the final four rules type
forwarding,
structured parallel composition, and the structural rules.

\ifalphalambda\else
One key design choice of our typing rules is that the processes in the multiplicative and the additive groups of rules are the same.
For example, the same send can be typed with~$A \sep B$ or with $A \land B$.
Their difference lays purely in the way they manage their available resources, possibly enabling or restricting the use of Rule~\ruleLabel{typ-struct} in other parts of the derivation.

\paragraph{Rules for multiplicative constructs.}
\fi

The type~$A \sep B$ is assigned to a session that sends a name of type~$A$ and continues as~$B$.
Rule~\ruleLabel{typ-sep-R} states that to \emph{provide} a session of type~$A \sep B$ on~$x$, a process must send on~$x$ a new name~$y$ and continue with a process providing a session of type~$A$ on~$y$ in parallel with a process providing the continuation session~$B$ on~$x$.
Rule~\ruleLabel{typ-sep-L} describes how to \emph{use} a session of type~$A \sep B$ on~$x$:
a process must receive on~$x$ a new name~$y$ which is to be used for the session of type~$A$, after which the process must provide the continuation session~$B$ on~$x$.

Rules~\ruleLabel{typ-wand-R} and~\ruleLabel{typ-wand-L} describe the type~$A \wand B$.
These rules are dual to the rules for $A \sep B$: providing $A \wand B$ requires a receive, and using it requires a send.

\newpage
Rule~\ruleLabel{typ-emp-R} states how to close a session of type~$\mOne$ using an empty send, followed by termination.
The dual Rule~\ruleLabel{typ-emp-L} uses the empty receive.
Note that Rule~\ruleLabel{typ-emp-R} requires the context to be~$\mEmpty$, effectively forcing processes to consume all the sessions they use before terminating.

\ifalphalambda\else
\paragraph{Rules for additive constructs.}
\fi

\ifalphalambda{}T\else{}As already mentioned, t\fi{}he rules for sessions of additive type are identical to the ones for multiplicative types, except that the latter (de)composes bunches using `$\,,\,$' while the former uses `$\,;\,$'.
In particular, the process interpretation of the rules is identical for both counterparts.
The difference has effect elsewhere, where the choice between `$\,;\,$' and `$\,,\,$' affects the possibility of using Rule~\ruleLabel{typ-struct} (explained last).

\ifalphalambda\else
\paragraph{Rules for disjunction.}
\fi

Disjunction types branching.
To provide on~$x$ a session of type~$A \lor B$, the process must select $\inl$/$\inr$ on~$x$ and continues by providing $A$/$B$, respectively.
Using a session of type~$A \lor B$ on~$x$ requires a branch on~$x$, where the left branch uses~$x$ as~$A$ and the right branch as~$B$.
\ifalphalambda\else
Curiously, there is no dual construct for disjunction in \BI, meaning that there is no way to type a selection on a channel that is being used, or a branch on a channel that is being provided.
There is no canonical way of adding such a dual construct; there are however extensions of \BI that incorporate one---see, e.g., \cite{thesis/Docherty19,book/Pym13,journal/sl/Brotherston12,journal/lmcs/BrotherstonC10,conf/csl/BrotherstonV15}.

\paragraph{Forwarders, cut, and structural rules.}
\fi

Rule~\ruleLabel{typ-fwd} types the forwarder~$\pFwd [x<>y]$ as providing a session of type~$A$ on~$x$ as a copycat of a session of the same type on~$y$ in the context.
Rule~\ruleLabel{typ-cut} connects processes $P$ and $Q$ along the channel $x$: $P$ must \emph{provide} a session of type $A$ on $x$, whereas $Q$ must \emph{use} the session of the same type on the same channel.

Rule~\ruleLabel{typ-bunch-equiv} closes typing under bunch equivalence (cf.\ \Cref{s:alphalambda:alphalambda:typeSys}).
Rule~\ruleLabel{typ-struct} extends indexed renaming (\ifalphalambda\Cref{d:alphalambda:idxRenaming}\else\Cref{d:piBI:idxRenaming}\fi) to bunches as follows.

\begin{definition}[Indexed Bunch Renaming]
    \ifalphalambda \label{d:alphalambda:idxBunchRenaming}
    \else \label{d:piBI:idxBunchRenaming} \fi
    Let~$\Delta$ be a bunch with $\fn(\Delta) = \{a,b,\dots,z\}$.
    Assuming $a_i,b_i,\dots,z_i \notin \fn(\Delta)$, we define $\idx{\Delta}{i} \deq \Delta \{ a_i/a,b_i/b,\ldots,z_i/z \},$ where $\Delta\theta$ is the bunch obtained by applying the substitution $\theta$ to all the leaves of~$\Delta$.
\end{definition}

\ifalphalambda\else
\begin{figure}[t]
    \begin{mathpar}
        \begin{bussproof}[typ-weaken]
            \bussAssume{
                \bunchCtx{\Gamma}[\Delta_2] \vdash P \typInf z:C
            }
            \bussAssume{
                \spvar = \map{x -> \emptyset | x \in \Delta_1}
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta_1 ; \Delta_2] \vdash \pSpw[\spvar] ; P \typInf z:C
            }
        \end{bussproof}
        \and
        \begin{bussproof}[typ-contract]
            \bussAssume{
                \bunchCtx{\Gamma}[\idx{\Delta}{1} ; \idx{\Delta}{2}] \vdash P \typInf z:C
            }
            \bussAssume{
                \spvar = \map{x -> x_1,x_2 | x \in \Delta}
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta] \vdash \pSpw[\spvar] ; P \typInf z:C
            }
        \end{bussproof}
    \end{mathpar}

    \caption{Usual presentations of weakening and contraction for \BI sequent calculi.}
    \label{f:piBI:weakenContractBI}
\end{figure}
\fi

Rule~\ruleLabel{typ-struct} subsumes and generalizes the two structural rules of weakening and contraction.
\ifalphalambda\else
To unpack the meaning of the rule, \Cref{f:piBI:weakenContractBI} gives rules for weakening and contraction as usually presented for \BI sequent calculi.
Rule~\ruleLabel{typ-weaken} discards the unused resources in~$\Delta_1$.
The process interpretation is a spawn that terminates the providers of sessions on channels in $\Delta_1$.
Rule~\ruleLabel{typ-contract} allows the duplication of the resources in~$\Delta$.
These resources need to be renamed to keep the names unique, hence the substitutions~$\idx{\Delta}{1}$ and $\idx{\Delta}{2}$ in the premise.
The process interpretation is again a spawn prefix that generates two indexed variants of each name in~$\Delta$, representing the duplicated resources.
For both rules, it is crucial that the affected bunches are combined using `$\,;\,$'.

Both Rule~\ruleLabel{typ-weaken} and~\ruleLabel{typ-contract} transform bunches according to the spawn binding of the involved names.
The idea behind Rule~\ruleLabel{typ-struct} is to generalize weakening and contraction, and allow more general spawn bindings.
As such, the rule combines in a single application a number of consecutive or independent applications of Rule~\ruleLabel{typ-weaken} and~\ruleLabel{typ-contract}.
\fi

To relate spawn bindings and their corresponding transformations of bunches, we define a \emph{spawn binding typing} judgment $\spvar \from \Delta_1 \tobunch \Delta_2$; the bottom of \Cref{f:piBI:typing} gives their rules.
The idea is to consider a binding~$\spvar$ as the merge of a sequence of bindings \mbox{$\spvar = \spvar_1 \spmerge \dots \spmerge \spvar_k$}, where each $\spvar_i$ is either a weakening or a contraction binding.
The weakening and contraction bindings are typed using Rules~\ruleLabel{spawn-weaken} and~\ruleLabel{spawn-contract}.
%</alphalamda:piBI:typing>
In case of contraction, when~$n=2$ we get pure contraction, when~$n>2$ it might represent a number of consecutive contractions applied to the same bunch; the corner case when~$n=1$ just renames the variables in the bunch, and might arise as the by-product of a contraction and a weakening (partially) canceling each other out.

Rules~\ruleLabel{spawn-weaken} and~\ruleLabel{spawn-contract} combined with Rule~\ruleLabel{typ-struct} offer a justification of the specialized Rules~\ruleLabel{typ-weaken} and~\ruleLabel{typ-contract}, respectively.
In the former case, the justification is direct.
The latter case holds for $n=2$, i.e., for pure contraction.

We wrap up the explanation of Rule~\ruleLabel{typ-struct} by giving an example typing derivation.

\begin{example}
    Consider the following process, with contraction and weakening in one:
    \[
        P \deq \pRes{x} \big( \pWait z() ; Q \|_x \pRes{y} ( \pClose y[] \|_y \pSpw[x->x_1,x_2;y->\emptyset] ; R ) \big)
    \]
    This process is well-typed, assuming $\Delta \vdash Q \typInf x:A$ and $\bunchCtx{\Gamma}[x_1:A ; x_2:A] \vdash R \typInf v:B$, as follows:
    \begin{align}
        & \begin{bussproof}
            \bussAx{
                \begin{array}{@{}r@{}}
                    \map{x->x_1,x_2} : \bunchCtx{\Gamma}[x:A ; y:\aOne]
                    \\
                    \tobunch \bunchCtx{\Gamma}[x_1:A ; x_2:A ; y:\aOne]
                \end{array}
            }
            \bussAx{
                \begin{array}{@{}r@{}}
                    \map{y->\emptyset} : \bunchCtx{\Gamma}[x_1:A ; x_2:A ; y:\aOne]
                    \\
                    \tobunch \bunchCtx{\Gamma}[x_1:A ; x_2:A]
                \end{array}
            }
            \bussBin{
                (\map{x->x_1,x_2} \spmerge \map{y->\emptyset}) : \bunchCtx{\Gamma}[x:A ; y:\aOne] \tobunch \bunchCtx{\Gamma}[x_1:A ; x_2:A]
            }
        \end{bussproof}
        \label{eq:piBI:x:spawn}
        \\
        & \begin{bussproof}
            \def\defaultHypSeparation{\hskip1ex}
            \bussAssume{
                \Delta \vdash Q \typInf x:A
            }
            \bussUn{
                \Delta , \mEmpty \vdash Q \typInf x:A
            }
            \bussUn{
                \Delta , z:\mOne \vdash \pWait z() ; Q \typInf x:A
            }
            \bussAx{
                \aEmpty \vdash \pClose y[] \typInf y:\aOne
            }
            \bussAssume{
                \bunchCtx{\Gamma}[x_1:A ; x_2:A] \vdash R \typInf v:B
            }
            \bussAssume{
                \eqref{eq:piBI:x:spawn}
            }
            \bussBin{
                \bunchCtx{\Gamma}[x:A ; y:\aOne] \begin{array}[t]{@{}l@{}}
                    \vdash \pSpw[x->x_1,x_2;y->\emptyset] ; R 
                    \\
                    \typInf v:B
                \end{array}
            }
            \bussBin{
                \bunchCtx{\Gamma}[x:A ; \aEmpty] \vdash \pRes{y} ( \pClose y[] \|_y \pSpw[x->x_1,x_2;y->\emptyset] ; R ) \typInf v:B
            }
            \bussUn{
                \bunchCtx{\Gamma}[x:A] \vdash \pRes{y} ( \pClose y[] \|_y \pSpw[x->x_1,x_2;y->\emptyset] ; R ) \typInf v:B
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta , z:\mOne] \vdash P \typInf v:B
            }
        \end{bussproof}
        \nonumber
    \end{align}
    Notice how the spawn binding must be split into a contracting and a weakening spawn binding to justify the transformation of the bunch.
\end{example}

It is worth noticing that the typing judgment $\spvar \from \Delta_1 \tobunch \Delta_2$ is not uniquely determined from~$\spvar$ and $\Delta_1$.
Hence, there is not always a unique derivation tree for a given judgment.
To recover unique typing, it should be sufficient to annotate all bindings with their respective types, including the $\spvar$ in the spawn prefixes.

\paragraph{Empty spawn.}

We briefly discuss a corner case:
according to the typing rules for spawn bindings, we can type the empty spawn $\pSpw[\emptyset]$.
It is tempting to add a structural congruence or reduction that removes it, since an empty spawn does not do much operationally:
an empty spawn can only propagate along cuts and silently merge into other spawns.
However, adding a reduction such as $\pSpw[\emptyset] ; P \redd P$ will cause complications because the empty spawn prefix, though operationally vacuous, can influence the typing.
An example is the following application of weakening:
\[
    \begin{bussproof}
        \bussAssume{
            \bunchCtx{\Gamma}[\aEmpty] \vdash P \typInf x:A
        }
        \bussUn{
            \bunchCtx{\Gamma}[\mEmpty] \vdash \pSpw[\emptyset] ; P \typInf x:A
        }
    \end{bussproof}
\]
Thus, such a reduction might slightly change the typing of a process across reductions, disproving type preservation.
This would unnecessarily complicate the system and, arguably, would not be in line with the Curry-Howard correspondence.

The empty spawn prefixes are but a minor annoyance: reductions can still happen behind spawn prefixes.
We do have to take extra care of the empty spawn when we show deadlock-freedom in \Cref{s:piBI:meta:tpdf} and weak normalization in \Cref{s:piBI:meta:wn}.
Next, we discuss additional examples.
%</piBI:piBI:typing>

\subsection{Examples and Comparisons}
\label{sec:examples-comparisons}

%<*piBI:piBI:examples>
The \piBI calculus is expressive enough to represent many useful concurrency patterns.
Here we show three significant examples and contrast \piBI's approach to related calculi.
Below we write $P \redd^k Q$ to mean that $P$ reduces to $Q$ in $k \geq 1$ consecutive steps.

\paragraph{Server and clients.}

Recall from \Cref{x:piBI:contraction} the process $R = \pRes{x} \big( \pWait z() ; P \| \pSpw[x->x_1,x_2] ; Q \big)$.
We can interpret $\pWait z() ; P$ as a server providing a service on~$x$ while relying on another server providing a service on~$z$, and the spawn as a request for two copies of the server to be used in~$Q$ on~$x_1$ and~$x_2$.

In \piDILL and \CP, servers and clients are expressed using replicated receives
$\pSrv x(y) ; P$, which upon receiving a channel~$y$ replicates~$P$ to provide its session on~$y$.
A client must then explicitly request a copy of the server by sending a fresh channel over~$x$.
The \piDILL analog of~$R$ would then be $R' \deq \pRes{u} \big( \pSrv u(x) ; \pCli* z[z'] ; \pWait z'() ; P \| \pCli* u[x_1] ; \pCli* u[x_2] ; Q \big)$.
In general, \piDILL's servers and clients can be expressed in \piBI by removing the replicated receives (i.e., $\pSrv x(y) ; P$ becomes $P \{ x/y \}$) and replacing request sends with spawns (i.e., $\pCli* x[x_1] ; Q$ becomes $\pSpw[x->x_1,x_2] ; Q \{ x_2/x \}$).

There is a crucial difference in the two models of servers:
in \piDILL, the server itself is responsible for creating a new instance of the session it provides, and thus needs to make sure that the sessions on which the new instance depends are themselves provided by servers.
In \piBI the responsibility for duplication lies with the client;
the server does not need to make special arrangements to allow for duplication, and its dependencies are duplicated on-the-fly by the spawn semantics.

The on-the-fly nature of spawn propagation makes the server/clients pattern more concurrent in \piBI than in \piDILL.
Suppose we connect~$R$ to a process providing~$z$.
The communication on~$z$ can take place before the spawn reduction, such that the spawn no longer needs to propagate to~$z$:
\[
    \pRes{z} ( \pClose z[] \| R ) \redd \pRes{x} ( P \| \pSpw[x->x_1,x_2] ; Q ).
\]
This is not possible in \piDILL: the replicated receive is blocking the communication on~$z$.

\paragraph{Failures.}

An important aspect of (distributed) programming is coping with failure.
For example, consider $P \deq \pIn x(y) ; \pWait x() ; \pOut* z[w] ; \big( \pFwd [w<>y] \| \pWait z() ; \pClose v[] \big)$, i.e., a process that receives a channel~$y$ over $x$ and forwards it over $z$.
Suppose that the process providing $x$ is unreliable, and might not be able to send the channel $y$.
This provider process indicates availability by a selection on $x$: left means availability and right means the converse.
We can then embed $P$ in a branch on $x$, where the right branch propagates the failure to forward a channel by means of spawn: $P' \deq \pBraLR x > {P}{\pWait x() ; \pSpw[z->\emptyset] ; \pClose v[]}$.
Let $\pIn z(q) ; R$ denote the process providing~$z$, which expects to receive a channel.
Indeed, in the following the behavior on $x$ is available:
\begin{align*}
    & \pRes{z} \Big( \pIn z(q) ; R \| \pRes{x} \big( \pSelL x ; \pOut* x[u] ; ( \pClose u[] \| \pClose x[] ) \| P' \big) \Big)
    \\
    & \redd^3 \pRes{z} \Big( \pIn z(q) ; R \| \pRes{u} \big( \pClose u[] \| \pOut* z[w] ; ( \pFwd [w<>u] \| \pWait z() ; \pClose v[] ) \big) \Big)
    \\
    & \redd^3 \pRes{u} \big( \pClose u[] \| \pRes{z} ( R \{ u/q \} \| \pWait z() ; \pClose v[] ) \big)
\end{align*}
In contrast, in the following example the behavior on $x$ is not available:
\[
    \pRes{z} \big( \pIn z(q) ; R \| \pRes{x} ( \pSelR{x} ; \pClose x[] \| P' ) \big) \redd^2 \pRes{z} ( \pIn z(q) ; R \| \pSpw[z->\emptyset] ; \pClose v[] ) \redd \pSpw[\emptyset] ; \pClose v[]
\]

The principle sketched in this example is inspired by the framework by \citet{conf/esop/CairesP17}, which supports communication primitives for non-deterministically (un)available behavior via a Curry-Howard interpretation of classical \LL with dedicated modalities.

\paragraph{Interaction between session delegation and spawn.}

Session delegation (also known as higher-order session communication) is the mechanism that enables the exchange of channels themselves over channels, dynamically changing the communication topology.
In \piBI, delegation interacts with spawn, in that changing process connections influences the propagation of spawn.
Let $P \deq \pRes{x} \big( \pOut* x[y] ; ( \pClose y[] \| \pClose x[] ) \| \pRes{z} ( \pIn x(w) ; \pWait x() ; \pWait w() ; \pClose z[] \| \pSpw[z->\emptyset] ; \pClose v[] ) )$.
From~$P$, we could either reduce the spawn prefix or synchronize on $x$.
If we first reduce the spawn, the spawn propagates to $x$:
\[
    P \redd \pRes{x} \big( \pOut* x[y] ; ( \pClose y[] \| \pClose x[] ) \| \pSpw[x->\emptyset] ; \pClose v[] \big).
\]
However, if we first synchronize on $x$, the spawn propagates to the delegated channel $y$:
\[
    P \redd^2 \pRes{y} \big( \pClose y[] \| \pRes{z} ( \pWait y() ; \pClose z[] \| \pSpw[z->\emptyset] ; \pClose v[] ) \big) \redd \pRes{y} ( \pClose y[] \| \pSpw[y->\emptyset] ; \pClose v[] ).
\]

\paragraph{Incomparability with \piDILL.}

As shown by~\citet{journal/jfp/OHearn03}, \DILL and \BI are incomparable.
Examining two canonical distinguishing examples can shed some light on the fundamental differences of the two logics, and their interpretations as session type systems.

As we remarked in \Cref{s:piBI:intro}, \DILL admits a ``number of uses'' interpretation, where linear resources have to be used exactly once.
This interpretation is not supported by \BI (cf.\ the example in \Cref{s:intro:contrib:lambda:alphalambda}):

In \piBI, it is possible to receive linearly (i.e., with~$\wand$) a session and use it twice.
The process $P \deq \pIn z(a) ; \pIn z(y) ; \pSpw[a->a_1,a_2] ; \pOut* y[a_1'] ; \big( \pFwd [a_1'<>a_1] \| \pOut* y[a_2'] ; ( \pFwd [a_2'<>a_2] \| \pFwd [z<>y] ) \big)$ can be typed as providing a session~$A \wand (A \to A \to B) \to B$ on~$x$:
\[
    \begin{bussproof}
        \bussAx{
            a_1:A \vdash \pFwd [a_1'<>a_1] \typInf a_1':A
        }
        \bussAx{
            a_2:A \vdash \pFwd [a_2'<>a_2] \typInf a_2':A
        }
        \bussAx{
            y:B \vdash \pFwd [z<>y] \typInf z:B
        }
        \bussBin{
            a_2:A ; y:A \to B \vdash \pOut* y[a_2'] ; ( \pFwd [a_2'<>a_2] \|
            \pFwd [z<>y] ) \typInf z : B
        }
        \bussBin{
            a_1:A ; a_2:A ; y:A \to A \to B \vdash \pOut* y[a_1'] ; \big( \pFwd [a_1'<>a_1] \| \pOut* y[a_2'] ; (\dots) \big) \typInf z:B
        }
        \bussUn{
            a:A ; y:A \to A \to B \vdash \pSpw[a->a_1,a_2] ; \big( \pOut* y[a_1'] ; (\dots) \big) \typInf z:B
        }
        \bussUn{
            a:A \vdash \pIn z(y) ; \pSpw[a->a_1,a_2] ; (\dots) \typInf z:(A \to A \to B) \to B
        }
        \bussUn{
            \mEmpty \vdash \pIn z(a) ; \pIn z(y) ; \pSpw[a->a_1,a_2] ; (\dots) \typInf z:A \wand (A \to A \to B) \to B
        }
    \end{bussproof}
\]
The process receives a single session of type~$A$ over~$z$
through linear receive.
The session on~$y$ anticipates~$A$ twice,
but allows these two $A$-typed sessions to share a common origin.
The process can thus spawn two copies of $a:A$
and use them to interact with~$y$.

The corresponding \LL proposition $A \lolli (A \to A \to B) \to B$ is not derivable:
\LL forbids using twice a resource obtained through linear receive.
However, the notion of linearity in \piBI has a more subtle reading:
it restricts the origin of sessions.
Above, the use of~$\to$ allows the duplication of the session at~$a$ into its copies~$a_1$ and~$a_2$;
this information about the ``origin'' of $a_1$ and $a_2$ is recorded in the bunch by the use of `$\,;\,$'.

On the other hand, there are types provable in \DILL that are not provable in \BI.
A simple example is $A \lolli B \vdash A \to B$, converting an implication from linear to non-linear.
A ``number of uses'' interpretation of the conversion makes sense:
$A \lolli B$ promises to use~$A$ exactly once to produce~$B$;
$A \to B$ declares to produce~$B$ using~$A$ an unspecified number of times, including exactly once.
The corresponding judgment~$A \wand B \vdash A \to B$ is not provable in \BI (and usable as typing derivation in \piBI).
Intuitively, this is because $A \to B$ allows~$A$ to be obtained with resources which share their origin with the resource~$A \wand B$;
however, $A \wand B$ can only be applied to resources that do not share its own origin.

\paragraph{The meaning of multiplicative and additive types.}

A natural question arises: if the process interpretation of multiplicatives and additives coincides, what is the difference in the types representing behaviorally?
The following example addresses the difference between linear and non-linear connectives;
in \ifthesis the publication derived from this thesis~\cite{conf/oopsla/FruminDHP22} \else \cref{sec:denot} \fi we formally elucidate this difference by giving a denotational semantics which allows tracking the \emph{origin} of sessions.

Assume an opaque base type~$\mbb{D}$ of data.
The type of a stylized database could be \mbox{$\sff{DB} \deq (\mbb{D} \to \sff{DB}) \land (\mbb{D} \land \sff{DB})$} where the first conjunct can receive some new data to overwrite the contents of the database (the `put' operation), and the second  would provide the current data stored in it (the `get' operation).
This is a recursive type, which is not currently supported by our calculus; for the purposes of this discussion, it is enough to consider some finite unfolding of the type (terminated with~$\aOne$).

Just by looking at the type $\sff{DB}$, we can identify possible interactions with the database.
A typical usage pattern of a resource~$\text{db}:\sff{DB}$ would be to receive the `put' and the `get' components and weaken the one we are not intending to use in the current step.
Imagine we want to put some $d:\mbb{D}$:
then we would weaken the `get', and send~$d$ over $\text{put}:(\mbb{D} \to \sff{DB})$ to obtain a continuation of type~$\sff{DB}$ that represents the updated database.

A second pattern of usage afforded by \piBI is to use contraction to spawn independent snapshots of the database.
For example, using contraction we can obtain, from $\text{db}:\sff{DB}$, a copy $\text{db}':\sff{DB}$.
From then on, the two copies can be mutated independently without interference.

Now consider two different \piBI processes, $P_{\sff{a}}$ and $P_{\sff{m}}$, with judgments:
\begin{mathpar}
    \text{db}_1:\sff{DB} ; \text{db}_2:\sff{DB} \vdash P_{\sff{a}} \typInf z:C
    \and
    \text{db}_1:\sff{DB} , \text{db}_2:\sff{DB} \vdash P_{\sff{m}} \typInf z:C
\end{mathpar}
$P_{\sff{a}}$ has access to two databases that are allowed to ``overlap'' since they are aggregated by a~`$\,;\,$'.
In contrast, $P_{\sff{m}}$ has access to two non-overlapping databases.
Here, ``overlapping'' has a subtle meaning:
it refers to the \emph{provenance} of the data in the two databases, rather than the stored value itself.
More concretely, imagine we interact, in both cases, with $\text{db}_1$ by weakening the `get', and with $\text{db}_2$ by weakening the `put' (and the continuation of `get'):
\begin{mathpar}
    \text{put}_1:\mbb{D} \to \sff{DB} ; \text{d}:\mbb{D}
    \vdash P'_{\sff{a}} \typInf z:C
    \and
    \text{put}_1:\mbb{D} \to \sff{DB} , \text{d}:\mbb{D}
    \vdash P'_{\sff{m}} \typInf z:C
\end{mathpar}
Process~$P'_{\sff{a}}$ is now allowed to send~$d$ on channel $\text{put}_1$, updating the database's value to~$d$, thus inducing a flow of information from $\text{db}_2$ to $\text{db}_1$.
This flow is however forbidden in the case of~$P'_{\sff{m}}$:
the data sent through $\text{put}_1$ needs to be obtained from a resource that is separated with it by `$\,;\,$' as per Rule~\ruleLabel{typ-impl-L}.
The fact that~$d$ is separated using~`$\,,\,$' fundamentally forbids it to flow into~$\text{put}_1$.

Now suppose $C = \mbb{D} * \mbb{D}$ and take $\sff{DB}$ to be the 1-unfolding of the recursive definition.
The typing of~$P_{\sff{m}}$ ensures that the two data values sent on the channel~$z$ would come one from~$\text{db}_1$ and the other from~$\text{db}_2$;
the combinations where two values taken from the same database are sent on $z$ are disallowed by typing.
\ifthesis\else
As we will see in \cref{ex:provenance,ex:db-reprise}, the denotational semantics developed in \cref{sec:denot} formally justifies these claims.
\fi
%</piBI:piBI:examples>




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> repos/pi-bi/paper/conclusion.tex <==
%!TEX root = main.tex
\section{Concluding Remarks and Future Perspectives}
\label{sec:conclusion}

%<*piBI:concl>
In this \ifthesis{}chapter\else{}paper\fi we present a fresh look at logical foundations for message-passing concurrency.
We have cast the essential principles of propositions-as-sessions, initially developed upon \LL, in the unexplored context of \BI.
We introduced the typed process calculus \piBI, explored its operational and type-theoretical contents, illustrated its expressiveness, and established the meta-theoretical framework needed to study the behavioral consequences of the \BI typing discipline for concurrency.

Our results unlock a number of enticing future directions.
First, because \piBI targets binary session types (between two parties) with synchronous communication, it would be interesting to study variants of \piBI with multiparty, asynchronous communication~\cite{journal/acm/HondaYC16,conf/popl/ScalasY19}.
An asynchronous version of \piBI could be defined by following the work of DeYoung \etal~\cite{conf/csl/DeYoungCPT12} to maximize concurrency.
Also, the works~\cite{conf/concur/CarboneMSY15,conf/concur/CarboneLMSW16,conf/forte/CairesP16} already provide insights on how to exploit \piBI to analyze multiparty protocols.

Second, variations and extensions of \BI could provide new insights.
For example, the ${!}A$ modality is not incompatible with \BI, and can be added to obtain a type ${!}A \simeq A * \dots * A$.
The intuitive interpretation is that the provider of~${!}A$ can create an instance of~$A$ from scratch, thus not sharing its origin with the other instances.
This new type would seem incomparable with the corresponding modality of \LL, which makes it interesting to study what interpretations could admit.
%</piBI:concl>

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> repos/pi-bi/paper/intro.tex <==
% !TeX root = ../../../main.tex
\section{Introduction}
\label{sec:intro}

%<*piBI:intro>
In this \ifthesis{}chapter\else{}paper\fi, we investigate a new point in the design space of session type systems for message-passing concurrent programs.
We identify the \emph{logic of bunched implications}~(\BI) of \citet{journal/bsl/OHearnP99} as a fruitful basis for an interpretation of the logic as a concurrent programming language, in the style of \emph{propositions-as-sessions}~\cite{conf/concur/CairesP10,conf/icfp/Wadler12}.
This leads to a treatment of \emph{non-linear resources} that is radically different from existing approaches based on Girard's linear logic~(\LL)~\cite{journal/tcs/Girard87,report/BarberP96}.
We propose \piBI, the first concurrent interpretation of \BI, and we study the behavioral properties enforced by typing, laying the meta-theoretical foundations needed\ifpiBI\else, and clarifying its relation to the other type-theoretic interpretations of \BI\fi.

\paragraph{Session types for message-passing concurrency.}

Writing concurrent programs is notoriously hard, as bugs might be caused by subtle undesired interactions between processes.
Statically enforcing the absence of bugs while allowing expressive concurrency patterns is important but difficult.
In the context of message-passing concurrency, type systems based on \emph{session types} provide an effective approach.
Session type systems enforce a communication structure between processes and channels, with the intent of (statically) ruling out races (as in, e.g., two threads sending messages over the same channel at the same time) and other undesirable behaviors, like deadlocks.
This communication structure is formulated at the type level.
For example, the session type $T={{!}\sff{int} . {?}\sff{str} . {!}\sff{bool} . \tEnd}$ (written in the syntax of \citet{journal/ic/Vasconcelos12}) describes a protocol that first outputs an integer (${!}\sff{int}$), then inputs a string~(${?}\sff{str}$), and finally outputs a boolean (${!}\sff{bool}$).
In session-based concurrency, types are assigned to channel names; this way, e.g.,
the assignment $x:T$ dictates that the communications on channel $x$ must adhere to the protocol described by~$T$.

The fundamental idea behind session types is that an assumption such as~$x:T$ is like a \emph{resource} that can be consumed and produced.
For example, sending an integer on the channel~$x$ consumes~$x:{!}\sff{int} . {?}\sff{string} . {!}\sff{bool} . \tEnd$ and produces a new resource $x:{?}\sff{string} . {!}\sff{bool} . \tEnd$, representing the expected continuation of the protocol.
Then, the coordinated use of channels requires a strict discipline on how resources can be consumed and produced:
it is unwise to allow multiple processes to access the same resource~$x:T$,
otherwise simultaneous concurrent outputs by different processes on the same channel will render the protocol invalid.
The type system is thus designed to enforce
that some resources, like those associated with channels, are \emph{linear}: they are consumed \emph{exactly once}.
By enforcing linearity of these resources, session type systems ensure that well-typed programs conform to the protocols encoded as types, and satisfy important correctness properties, such as deadlock-freedom.

\paragraph{Propositions-as-sessions.}

A central theme in this \ifthesis thesis \else paper \fi is how logical foundations can effectively inform the design of expressive type disciplines for programs.
In the realm of functional programming languages,
such logical foundations have long been understood via type systems obtained
through strong Curry-Howard correspondences with known logical proof systems
(e.g., the correspondence between the simply-typed \lamcalc and intuitionistic propositional logic).
For concurrent languages, on the other hand, such correspondences have been more elusive.
Indeed, although the original works on session types by Honda \etal~\cite{conf/concur/Honda93,conf/esop/HondaVK98} feature an unmistakable influence of \LL in their formulation, the central question of establishing firm logical foundations for session types remained open until relatively recently.
The first breakthroughs were the logical correspondences based on the concurrent languages \piDILL~\cite{conf/concur/CairesP10} and \CP~\cite{conf/icfp/Wadler12} (based on intuitionistic \LL and classical \LL, respectively).
These works define a bidirectional correspondence, in the style of Curry-Howard, which allows us to interpret propositions as session types (protocols), proofs as \picalc processes, and \ruleLabel{cut}-elimination as process communication.
These correspondences are often collectively referred to as \emph{propositions-as-sessions}.

Intensely studied in the last decade, the line of work on propositions-as-sessions provides a principled justification to a linear typing discipline.
These correspondences also clarify our understanding of the status of \emph{non-linear} resources, which do not obey resource consumption considerations.
Non-linear resources, such as mutable references, client/server channels, and shared databases, are commonplace in practical programs and systems.
Disciplining non-linear resources is challenging, because there is a tension between flexibility and correctness: ideally, one would like to increase the range of (typable) programs that can be written, while ensuring that such programs treat non-linear resources consistently.

\LL allows for a controlled treatment of non-linear resources through the modality~${!}A$.
Within propositions-as-sessions, the idea is that a session of type ${!}A$ represents a server providing a session of type $A$ to its clients, and the server itself can be duplicated or dropped.
Those features---being able to replicate or drop a session---are achieved through the usage of \emph{structural rules} in the sequent calculus, specifically the rules of contraction and weakening, which are restricted to propositions of the form ${!}A$.
A series of recent works have explored quite varied ways of going beyond this treatment of non-linear resources: they have put forward concepts such as \emph{manifest sharing}~\cite{conf/icfp/BalzerP17,conf/esop/BalzerTP19}, dedicated frameworks such as \emph{client-server logic}~\cite{conf/icfp/QianKB21}, and specific constructs for non-deterministic, fail-prone channels~\cite{conf/esop/CairesP17}.

\paragraph{The logic of bunched implications.}

At their heart, the aforementioned works propose different ways of treating non-linear resources through modalities.
Relaxing linearity through a modality allows a clean separation between the worlds of linear and non-linear resources.
This approach relies on rules that act as ``interfaces'' between the two worlds, allowing conversions  between linear and non-linear types only under controlled circumstances.

However, modalities are not the only way in which substructural logics can integrate non-linear resources.
A very prominent alternative is provided by the logic of bunched implications~(\BI) of \citet{journal/bsl/OHearnP99}.
\BI embeds the pure linear core of \LL as multiplicative conjunction~$\sep$ and implication~$\wand$, but extends it by introducing additive conjunction~$\land$ and implication~$\to$, which are treated non-linearly.
\BI can thus be thought of as enabling the free combination of linear and non-linear resources in a single coherent logic.

The result is a logic which admits an interpretation of linearity that is enticingly different from \LL.
Conceptually, \LL admits a ``number of uses'' interpretation, where types can specify \emph{how many times a resource should be used}: exactly once for linear resources, any number of times for~${!}A$ resources.
On the contrary, \BI admits an ``ownership'' interpretation~\cite{journal/tcs/PymOY04}, which focuses on \emph{who has access to which resources}.

The ownership interpretation has positioned \BI as the logic of choice for program logics for reasoning about stateful and concurrent programs, under the umbrella of (Concurrent) Separation Logic (see, e.g., the surveys by O'Hearn and Brookes~\cite{journal/acm/OHearn19,journal/siglog/BrookesO16}).
While separation logic has received significant attention, the same cannot be said about type-theoretic interpretations of \BI as a type system for concurrency.
To our knowledge, the only type-theoretic investigation into the (proof theory of) \BI has been the \alcalc~\cite{journal/jfp/OHearn03}---a \lamcalc arising from the natural deduction presentation of \BI---and its variations \cite{conf/icalp/Atkey04,journal/mscs/CollinsonPR08}.
\ifpiBI
The \alcalc and its connections to the work presented in this chapter are further explored in \Cref{c:alphalambda}.

\paragraph{The key idea.}

Here we propose \piBI: the first process calculus for the propositions-as-sessions and processes-as-proofs interpretation of \BI, based on its sequent calculus formulation.
The result is an expressive concurrent calculus with a new mechanism to handle non-linear resources, which satisfies important behavioral properties, derived from a tight correspondence with \BI's proof theory.
The central novelty of \piBI is a process interpretation of the structural rules, which closely follows the proof theory of \BI.

Consider the case of contraction/duplication.
Given a session $x:A$, how can we duplicate it into sessions $x_1:A$ and $x_2:A$?
The difficulty here is that after duplication, the two assumptions might be used differently and asynchronously.
We conclude that the actual process implementing those sessions in the current evaluation context needs to be duplicated, such that two independent processes can provide the duplicated sessions.
This ``on demand non-local replication'' of a process in the evaluation context is not something supported natively by the \picalc.
We propose a new process construct, a prefix dubbed \emph{spawn}, which achieves this.

We illustrate the spawn prefix with a simple example.
Let $P$ and $Q$ be two processes, with $P$ providing a service on the channel $x$, and $Q$ requiring two copies of the service.
The spawn prefix $\pSpw[x->x_1,x_2]$ denotes a request to the environment to duplicate the service on~$x$ into copies on the new channels $x_1$ and $x_2$.
Then, $\pSpw[x->x_1,x_2] ; Q$ is a process that first performs the request and then behaves as $Q$.
The composition of these processes is denoted $\pRes{x} ( P \| \pSpw[x->x_1,x_2] ; Q )$, where `$\,\|\,$' and `$\,\pRes{x}\,$' stand for parallel composition and restriction on $x$, respectively.

In the reduction semantics of \piBI, obtained from the proof theory of \BI, the composed process reduces as follows:
\[
    \pRes{x} ( P \| \pSpw[x->x_1,x_2] ; Q ) \redd \pRes{x_1} \big( P \{ x_1/x \} \| \pRes{x_2} ( P \{ x_2/x \} \| Q ) \big)
\]
This way, the duplication request leads to the composition of two copies of $P$ (each with an appropriate substitution $\{ x_i/x \}$) with the process $Q$ on channels $x_1$ and $x_2$, as desired.

The behavior of the spawn prefix is determined by the context in which it is executed and it communicates with the run-time system to achieve contraction or weakening.
This mechanism reminds us of horizontal scaling in cloud computing, with the spawn prefix playing the role of middleware: it requests the runtime environment to scale up/down a particular resource.
For example, a load balancer might determine that in a certain situation the execution environment has to provide an additional snapshot of a Docker container, and route part of the environment's requests to it.

As we will see, spawn reductions involve the propagation of the effects of duplicating processes (such as $P$ above);
we give the full definition and illustrate it further in \Cref{s:piBI:piBI}.

\paragraph{Contributions.}

As mentioned, the spawn prefix provides a direct interpretation of the structural rules in the design of the type system, adopting \BI as the underlying logic.
The resulting system is significantly expressive and yet different from  systems derived from propositions-as-sessions, which is not so surprising.
As logics, \BI and \LL are \emph{incomparable}: there are provable formulas of \LL that are not provable in \BI, and vice versa.
As such, an immediate question is whether \piBI satisfies the expected meta-theoretical properties for session-typed processes: \emph{type preservation} and \emph{deadlock-freedom}.
The key difficulty is that the semantics of the spawn prefix is fundamentally \emph{non-local}---it depends on its execution context.
\ifpiBI The main contribution of this chapter is that
\else As a \textbf{first contribution}, \fi
we show that type preservation and deadlock-freedom hold for \piBI; moreover, we prove \emph{weak normalization}, which further justifies the semantics of spawn prefixes.

\ifpiBI\else
In addition to these meta-theoretical properties, an essential ingredient in the propositions-as-sessions research program is defined by concurrent interpretations  of (typed) functional calculi, in the spirit of Milner's seminal work on \emph{functions-as-processes}~\cite{milner:1992}.
As already mentioned, the only prior type-theoretic interpretation of \BI is the (sequential) calculus \alcalc~\cite{ohearn:2003}.
As a \textbf{second contribution}, we define a translation from  \alcalc into \piBI, and prove that it correctly preserves and reflects the operational semantics of terms and processes, respectively.


While insightful and novel, the operational semantics of  \piBI and the translation of the \alcalc do not offer us a direct insight into the meaning of and difference between the types in our system (as is the case in the \alcalc).
A natural question is: what is the difference between multiplicative conjunction $\ast$ and additive conjunction $\wedge$ in \piBI?
As an answer to this question, our \textbf{third contribution} is a \emph{denotational semantics} for \piBI, which interprets processes as functions and describes types in terms of ``provenance tracking''.

Intuitively, our denotational semantics considers that duplication through a spawn prefix generates typed processes with the same provenance.
This notion of provenance then allows us to precisely distinguish between $\ast$ and $\wedge$: in a process with a session of type $A \ast B$ the sub-processes providing sessions $A$ and $B$ have a \emph{different origin}, a property that may not necessarily hold for processes with sessions of type $A \wedge B$.
This is possible because the provenance information can be reconstructed from a typing derivation, and it is made evident through the denotational semantics.

In addition to providing a semantic meaning to types, the denotational semantics is sound with regard to \emph{observational equivalence}.
Two processes are observationally equivalent if no other process can (operationally) distinguish between them.
Establishing observational equivalence of programs directly is hard, because it involves reasoning about process behavior under arbitrary contexts.
On the other hand, a denotational semantics provides a direct way of establishing equivalence: if two processes have the same denotation, then they are observationally equivalent.
As an application of the denotational semantics, we frame the operational correspondence for the \alcalc mentioned above in terms of observational equivalence.
\fi

\paragraph{Outline.}

The rest of the \ifthesis chapter \else paper \fi is organized as follows.
\Cref{s:piBI:piBI} presents the syntax, semantics, and type system of \piBI, and illustrates its expressivity.
In \Cref{s:piBI:meta}, we establish key meta-theoretical properties of typable processes: type preservation, deadlock freedom, and weak normalization.
\ifpiBI\else
We formally connect the  \alcalc to \piBI by  defining a translation and proving  operational correspondence for it in \Cref{sec:translation}.
We define the denotational semantics for \piBI processes, define observational equivalence, and formally relate the two in \Cref{sec:denot}.
\fi
We discuss further related work in \Cref{s:piBI:rw} and conclude in \Cref{s:piBI:concl}.
The omitted technical details can be found in \ifappendix \Cref{ac:piBI} \else \cite{thesis/vdHeuvel24ex} \fi.
%</piBI:intro>

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> repos/pi-bi/paper/meta.tex <==
% !TeX root = ../../../main.tex
\section{Meta-theoretical Properties}
\label{sec:meta}

%<*piBI:meta>
A distinguishing feature of the propositions-as-sessions approach is that the main meta-theoretical properties of session-typed processes (e.g., type preservation and deadlock-freedom) follow immediately from the cut elimination property in the underlying logic.
In this section we show that \piBI satisfies these properties, which serves to validate the appropriateness of our interpretation.
We consider type preservation and deadlock-freedom, but also \emph{weak normalization}.
\ifappendix \Cref{ac:piBI} \else \cite{thesis/vdHeuvel24ex} \fi gives additional properties and detailed proofs.
%</piBI:meta>

\subsection{Type Preservation and Deadlock-Freedom}
\label{sec:type_preservation_and_deadlock_freedom}

%<*piBI:meta:tpdf>
Essential correctness properties in session-based concurrency are that (i)~processes correctly implement the sessions specified by its types (session fidelity) and (ii)~there are no communication errors or mismatches (communication safety).
Both these properties follow from the \emph{type preservation} property, which ensures that typing is consistent across structural congruence and reduction.

\begin{restatable}[Type Preservation]{theorem}{tPiBITp}
    \label{t:piBI:tp}
    Assume $\Delta \vdash P \typInf x:C$.
    If $P \congr Q$ or $P \redd Q$, then $\Delta \vdash Q \typInf x:C$.
\end{restatable}

\begin{sketch}
    As a consequence of the tight correspondence between \piBI and the proof theory of \BI: structural congruence and reduction correspond to proof equivalences and (principal) cut reductions in the \BI sequent calculus (see \ifappendix \Cref{as:piBI:tp} \else \cite{thesis/vdHeuvel24ex} \fi for details).
\end{sketch}

Another important correctness property is \emph{deadlock-freedom}: the guarantee that processes never get stuck waiting on pending communications.
In general, deadlock-freedom holds for well-typed \piBI processes where all names are bound, except for the provided name, which must be used only to close a session.
Any process satisfying these typing conditions can then either reduce, or it is \emph{inactive}: only the closing of the session on the provided name is left, possibly prefixed by an empty spawn.
Because of bunches, a process with all names bound but one is typable in more ways than just under an empty typing context:

\begin{definition}[Empty Bunch]
    \label{d:piBI:emptyBunch}
    An \emph{empty bunch}~$\Sigma$ is a bunch such that
    $\fn(\Sigma) = \emptyset$.
    Equivalently, a bunch is empty if each of its leaves is $\mEmpty$ or $\aEmpty$.
\end{definition}

\begin{restatable}[Deadlock-freedom]{theorem}{tPiBIDf}
    \label{t:piBI:df}
    Given an empty bunch $\Sigma$, if $\Sigma \vdash P \typInf z:A$ with $A \in \{\mOne,\aOne\}$, then either (i)~$P \congr \pClose z[]$, or (ii)~$P \congr \pSpw[\emptyset] ; \pClose z[]$, or (iii)~there exists $S$ such that $P \redd S$.
\end{restatable}

\begin{sketch}
    The \piBI interpretation of Rule~\ruleLabel{typ-cut} combines restriction and parallel, ensuring that parallel processes never share more than one channel and thus preventing processes such as $\pRes{x} \pRes{y} \big( \pWait y() ; \pClose x[] \| \pWait x() ; \pClose y[] \big)$ where the subprocesses are stuck waiting for each other.
    The proof follows from a property that we call \emph{progress}, which  ensures that processes of a given syntactical shape can reduce.
    This reduces the proof to showing that processes typable under empty bunches are in the right syntactical shape to invoke progress.
\end{sketch}

The property stated above is an important feature of \piBI derived from its logical origin.
Although weak by itself, the progress property in the proof of deadlock-freedom is useful in providing a reduction strategy for practical implementations of \piBI.
%</piBI:meta:tpdf>

\subsection{Weak Normalization}
\label{sec:weak_normalization}

%<*piBI:meta:wn>
We now turn our attention to proving that our calculus is weakly normalizing.
That is, for every process $P$ there exists some process $Q$ such that $P \redd* Q \nredd$.
\ifthesis
In the publication derived from this chapter~\cite{conf/oopsla/FruminDHP22}, this result is of independent interest, as it is used to show soundness of denotational semantics.
\else
This is a result of independent interest, which we will use to show soundness of denotational semantics in \Cref{sec:denot}.
\fi
\ifthesis\else The normalization proof that we give here is of combinatorial nature. \fi
We outline the main ideas; details are given in \ifappendix \Cref{as:piBI:wn}\else \cite{thesis/vdHeuvel24ex}\fi.

Given a process $P$, what kind of reductions can $P$ make, and can we come up with some kind of measure that would strictly decrease and disallow infinite reduction sequences?
If we did not have the spawn prefix, then the answer to this problem would be simple: each reduction is an instance of communication (or a forwarder reduction), which decreases the total number of communication prefixes in the process.
However, in presence of spawn, counting the total number of prefixes does not work.
For example, consider the following reduction, where $\fn(R) = \{x,y\}$,
\begin{align}
    \pRes{x} \big( R \| \pSpw[x->x_1,x_2] ; Q \big)
    \redd
    \pSpw[y->y_1,y_2] ; \pRes{x_1} \big( \idx{R}{1} \| \pRes{x_2} ( \idx{R}{2} \| Q ) \big).
    \label{eq:piBI:dummySpawnRed}
\end{align}
In this reduction, the prefixes in the sub-process $R$ get duplicated, so the total number of prefixes increases.
What has also changed is that the spawn prefix $\pSpw[x->x_1,x_2]$ turned into the prefix $\pSpw[y->y_1,y_2]$ with a larger scope.
As a result, the communication prefixes in $Q$ went from being guarded directly by $\pSpw[x->x_1,x_2]$, to being guarded by a prefix $\pSpw[y->y_1,y_2]$, with the latter prefix being ``smaller'' in the sense that it is closer to the top-level of the process.

Furthermore, if the reduction~\eqref{eq:piBI:dummySpawnRed} occurs in some context $\evalCtx{K}$, then we can use Rules~\ruleLabel{red-spawn-R} and~\ruleLabel{red-spawn-L} to actually propagate the spawn prefix to the top-level:
\begin{align}
    \evalCtx[\big]{K}[\pRes{x} ( R \| \pSpw[x->x_1,x_2] ; Q )]
    & \redd
    \evalCtx[\big]{K}[\pSpw[y->y_1,y_2] ; \pRes{x_1} \big( \idx{R}{1} \| \pRes{x_2} ( \idx{R}{2} \| Q ) \big)]
    \label{eq:piBI:dummySpawnRed2}
    \\
    & \redd*
    \pSpw[y->y_1,y_2] ; \evalCtx{K}[\pRes{x_1} \big( \idx{R}{1} \| \pRes{x_2} ( \idx{R}{2} \| Q ) \big)],
    \nonumber
\end{align}
assuming $\evalCtx{K}$ has no other spawn prefixes that would interfere with $\pSpw[y->y_1,y_2]$.

Following this observation, the trick is to stratify the number of prefixes at each $\rho$-\emph{depth}, which is the number of spawn prefixes behind which the said prefix occurs.
So, if we examine the previous reduction sequence~\eqref{eq:piBI:dummySpawnRed2} and ignore the top-level spawn prefix, the communication prefixes in $Q$ went from being at depth $n+1$ to being at depth $n$.
While the number of prefixes at depth $n$ has increased, the number of prefixes at depth $n+1$ has decreased.
This suggests that we should consider a progress measure that aggregates the number of prefixes, giving more weight to prefixes at greater $\rho$-depths.

Our reduction strategy for weak normalization is then as follows.
If a process can perform a communication reduction or a forwarder reduction, then we do exactly that reduction.
If a process can only perform a reduction that involves a spawn prefix, then we
\begin{enumerate}
    \item select an (active) spawn prefix with the least depth;
    \item perform the spawn reduction;
    \item propagate the newly created spawn prefix to the very top-level, merging it with other spawn prefixes along the way.
\end{enumerate}

To show that this reduction strategy terminates, we adopt a measuring function that assigns to each process $P$ a finite mapping $\mu(P) \from \mbb{N} \to \mbb{N}$ assigning to each number $n$ the number of communication prefixes at depth $n$ and above.
In order to handle the special case of a top-level prefix, the measure function simply skips it, i.e. $\mu(\pSpw[\spvar] ; P) = \mu(P)$.
We then define an ordering $\skelLt$ on such mappings which prioritizes the number of prefixes at greater depths, and show that it is well-founded.

Then, we argue that each clause of our reduction strategy strictly decreases the measure.
Since the relation $\skelLt$ is well-founded, it guarantees that our strategy terminates.
If we perform a communication reduction, then the number of communication prefixes at a given depth decreases, which strictly decreases the measure.
If we perform a spawn reduction, then the number of prefixes at some depth $n+1$ might decrease, but the number of prefixes at depth $n$ might increase, because of the propagated spawn prefix.
In this case, we keep propagating the spawn prefix to the top-level as much as possible, to be skipped by the measure function at the top-level (possibly merging it with an existing top-level spawn).
In both cases, the maximal prefix depth of the process decreases, which results in a strictly decreased measure.

\ifthesis\else Due to space limitations, we refer the interested reader to \appendixref{appendix:sec:wn} for the full details. \fi

\begin{restatable}[Weak Normalization]{theorem}{tPiBIWn}
    \label{t:piBI:wn}
    If $\Delta \vdash P \typInf z:A$ is a typed process, then $P$ is weakly normalizing, i.e., there exists some $Q$ such that $P \redd* Q \nredd$.
\end{restatable}

\Cref{t:piBI:wn} captures the fact that, starting from a process $P$, different reductions may apply, or that there might be multiple spawns that can be brought to the top-most level.

Strictly speaking, we do not require well-typedness assumptions for establishing weak normalization; this property is enforced by the reduction semantics.
This is a pleasant consequence of our design for the syntax of processes, which already incorporates some of the structure imposed by typing; this structure is then preserved via the correspondence between commuting conversions and reductions.
As such, even the untyped processes are ``well-scoped'' in the sense that they conform to the tree-like structure typical of session-based interpretations of intuitionistic logics.

\Cref{t:piBI:wn} is related to cut-elimination in \BI, but the two theorems are not equivalent.
The main discrepancy lies in the fact that not all cut-reductions in \BI correspond to reductions of \piBI processes;
process reductions correspond to reductions of cuts which are not guarded by an input or an output prefix.
Consecutively, we cannot directly adopt the usual cut-elimination procedure for \BI~\cite{conf/tase/ArisakaQ12} for the purposes of showing weak normalization.
%</piBI:meta:wn>




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> repos/pi-bi/paper/relwork.tex <==
% !TeX root = ../../../main.tex
\section{Related Work}
\label{sec:rel_work}

%<*piBI:rw>
We have already discussed some of the most closely related works, and we have given some comparisons with previous works by means of examples in \Cref{s:piBI:piBI:examples}.
Here we discuss other related literature along several dimensions.

\paragraph{\BI and process calculi.}

To our knowledge, the work of \citet{journal/tcs/AndersonP16} is the only prior work that connects \BI with process calculi.
Their technical approach and results are very different from ours.
They introduce a process calculus (a synchronous CCS) with an explicit representation of (bunched) resources, in which processes and resources evolve hand-in-hand.
Rather than a typed framework for processes or an interpretation in the style of propositions-as-types, they use a logic related to \BI to specify rich properties of processes, in the style of Hennessy-Milner logic.

\paragraph{\BI and Curry-Howard correspondence.}

%<*alphalambda:rw>
The works of \citet{journal/jfp/OHearn03} and \citet{book/Pym13} are, to our knowledge, the only prior investigations into (non-concurrent) Curry-Howard correspondences based on \BI.
These works were later extended to cover polymorphism~\cite{journal/mscs/CollinsonPR08} and store with strong update~\cite{journal/entcs/BerdineO07}.
An extension $\lambda_{\sff{sep}}$ of an affine version of the \alcalc with a more fine-grained notion of separation was studied by \citet{conf/icalp/Atkey04,thesis/Atkey06}.
%</alphalambda:rw>

\paragraph{Previous works on propositions-as-sessions.}

Starting with the works by~\citet{conf/concur/CairesP10} and \citet{conf/icfp/Wadler12}, the line of work on propositions-as-sessions has exclusively relied on (variants of) \LL, which is incomparable to \BI; this immediately separates those prior works from our novel approach based on \BI.

Our work adapts to the \BI setting key design principles in~\cite{conf/concur/CairesP10,conf/icfp/Wadler12}: the interpretation of multiplicative conjunction as output, linear implication as input, and the interpretation of `cut' as the coalescing of restriction and parallel composition.
Those works use input-guarded replication to accommodate non-linear sessions, typed with the modality ${!}A$; in contrast, \piBI handles structural principles directly with the new spawn prefix.

Our adaptation is novel and non-trivial, and cannot be derived from prior interpretations based on \LL.
Still, certain aspects of \piBI bear high-level similarities with elements from those interpretations.
The semantics of our spawn prefix borrows inspiration from the treatment of aliases in Pruiksma and Pfenning's interpretation of asynchronous binary sessions based on adjoint logic, in which structural rules are controlled via modalities~\cite{journal/jlamp/PruiksmaP20}.
Thanks to spawn binders (\Cref{d:piBI:spawnEnv}), our semantics explicitly handles duplication and disposal of services; this is similar in spirit to the syntax and semantics of replicated servers in HCP, an interpretation based on a hypersequent presentation of classical \LL~\cite{conf/popl/KokkeMP19}.
The behavioral theory of HCP consists of a labeled transition semantics for processes, a denotational semantics for processes, and a full abstraction result.
The work of~\citet{conf/icfp/QianKB21} extends linear logic with coexponentials with the aim of capturing client-server interactions not expressible in preceding interpretations of linear logic.
Precise comparisons between the expressivity of such interactions and the connection patterns enabled by our spawn prefix remains to be determined.
Concerning failures, as discussed in \Cref{s:piBI:piBI:examples}, the work of Fowler \etal~\cite{conf/popl/FowlerLMD19} develops a linear functional language with asynchronous communication and support for failure handling, closely related to Wadler's \CP.
%</piBI:rw>

\paragraph{Observational equivalence}
Observational equivalence compares the behaviour of two processes
in \emph{every} (well-typed) program context.
This universal quantification makes  direct proofs of equivalence
very hard and non-compositional.
Observational equivalence is therefore usually established
using more compositional methods that do not involve reasoning
about a program in a context.
Examples of these methods are bisimulations and logical relations; in the session-typed setting, such methods have been addressed in~\cite{kouzapas.yoshida.honda:2011} and \cite{caires.perez.pfenning.toninho:2013,perez.etal:2014,DBLP:conf/esop/Atkey17,derakhshan.balzer.jia:2021}, respectively.
In \cref{sec:denot} we followed an approach based on denotational semantics, exploiting a canonical construction.
Our denotational semantics also serves to
%\seehere[bas]{dual}\bas*{Do you mean ``added'' or something similar?}
elucidate the difference between
the additive and multiplicative types.
Our proof of adequacy of the denotational semantics
for proving observational equivalence (\cref{thm:denot_equiv_sound})
relies on weak normalization (\cref{thm:weak_norm}).
In extensions of \piBI for which weak normalization does not hold,
our proof strategy would need to be revised.
Recent work on denotational semantics and logical relations for session-typed languages~\cite{derakhshan.balzer.jia:2021,Kavanagh22}
could provide the basis for handling such extensions.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> repos/pi-bi/paper/translation.tex <==
% !TeX root = ../../../main.tex
\section{Translating the \texorpdfstring{\alcalc}{alpha-lambda-calculus} into \texorpdfstring{\piBI}{piBI}}
\label{sec:translation}
The \alcalc is a functional calculus that is in a Curry-Howard correspondence with the natural deduction representation of \BI~\cite{ohearn:2003,pym:2002}.
%<*alphalambda:trans>
Here, we develop a type-preserving translation from the \alcalc to \piBI, and establish its correctness in a very strong sense: the translation satisfies an \emph{operational correspondence} property, which asserts how reductions in the source and target calculi are preserved and reflected (\Cref{t:alphalambda:completeness,t:alphalambda:soundness}, respectively).
%</alphalambda:trans>

\subsection{The \texorpdfstring{\alcalc}{Alpha-Lambda-Calculus} and Its Translation into \texorpdfstring{\piBI}{piBI}}
%
\begin{mathfig}[\small]
\adjustfigure
\rulesection*{Type system}
\input{figures/alcalc_short}
\rulesection{Reduction rules}
\input{figures/alcalc_red_short}
\caption{Selected rules of the type system and reduction rules for the \alcalc.}
\label{fig:alpha_lambda_typing}
\end{mathfig}
%
%
We first recall the statics and dynamics of the \alcalc.
Our formulation of the type system is based on the presentations by~\citet{ohearn:2003} and \citet[Chapter 2]{pym:2002}.

%<*alphalambda:alphalambda:syntax>
We use $M,N,L,\ldots$ for terms, and $a,b,c,\ldots,x,y,z,\ldots$ for variables.
\ifthesis

\begin{figure}[t]
    \begin{align*}
        M,N,L &
        \begin{array}[t]{@{}l@{}lr@{\kern2em}l@{\kern1em}lr@{}}
            {} ::= {} &
            x & \text{variable}
            \\ \sepr* &
            \lam x . M & \text{abstraction}
            & \sepr &
            M\ N & \text{application}
            \\ \sepr* &
            \alpha x . M & \text{abstraction}
            & \sepr &
            M \at N & \text{application}
            \\ \sepr* &
            \mUnit & \text{unit}
            & \sepr &
            \tLet \mUnit = M \tIn N & \text{unit-let}
            \\ \sepr* &
            \aUnit & \text{unit}
            & \sepr &
            \tLet \aUnit = M \tIn N  & \text{unit-let}
            \\ \sepr* &
            \<M,N\> & \text{pair}
            & \sepr &
            \tLet \<x,y\> = M \tIn N & \text{pair-let}
            \\ \sepr* &
            (M,N) & \text{pair}
            & \sepr &
            \pi_i M & \text{projection}
            \\ \sepr* &
            \tSel_i(N) & \text{selection}
            & \sepr &
            \tCase M \tOf \{ 1(x_1):N , 2(x_2):L \} & \text{branch}
        \end{array}
    \end{align*}

    \caption{Syntax of the \alcalc (\Cref{d:alphalambda:alphalambda:syntax}).}\label{f:alphalambda:alphalambda:syntax}
\end{figure}

\begin{definition}[Syntax of the \alamcalc]
    \label{d:alphalambda:alphalambda:syntax}
    \Cref{f:alphalambda:alphalambda:syntax} gives the syntax of the \alcalc.
\end{definition}

The \alcalc is based on the \lamcalc, but (almost) all of its constructs come in two variants: one multiplicative and one additive.
Multiplicative (resp.\ additive) abstraction `$\lam x . M$' (resp.\ `$\alpha x . M$') is to be used with the corresponding application `$M\ N$' (resp.\ `$M \at N$').
The multiplicative (resp.\ additive) unit `$\mUnit$' (resp.\ `$\aUnit$') is to be used with the corresponding unit-let `$\tLet \mUnit = M \tIn N$' (resp.\ `$\tLet \aUnit = M \tIn N$').
Multiplicative pairs `$\<M,N\>$' can be ``unpacked'' with the pair-let construct `$\tLet \<x,y\> = M \tIn N$', while additive pairs `$(M,N)$' can be projected with `$\pi_i(M)$' (where $i \in \{1,2\}$).
Selection `$\tSel_i(N)$' and branching `$\tCase M \tOf \{1(x_1):N , 2(x_2):L\}$' appear in one variant only.

\else
The \alcalc is based on the \lamcalc, but with two separate kinds of function binders: $\lam x . M$ with its corresponding function application $M\ N$ for the magic wand $A \wand B$, and $\alpha x . M$ with its corresponding function application $M \at N$ for the intuitionistic implication $A \to B$.
Selected typing rules are given in the top of \Cref{{fig:alpha_lambda_typing}}; the full type system can be found in \appendixref{sec:appendix:translation}.
\fi

We write $\fv(M)$ to denote the free variables of $M$.
As usual, substitution of a term $N$ for a variable $x$ in a term $M$ is denoted $M \{ N/x \}$.
We write $M \{ N_1/x_1,\ldots,N_n/x_n \}$ for the sequence of substitutions $M \{ N_1/x_1 \} \ldots \{ N_n/x_n \}$.
%</alphalambda:alphalambda:syntax>

%<*alphalambda:alphalambda:reduction>
The reduction semantics of the \alcalc, denoted $M \aredd N$, follows a call-by-name  strategy for the \lamcalc\ifthesis\else, extended to cover two kinds of function binders\fi.
\ifthesis
\Cref{f:alphalambda:reduction} gives the rules to derive reductions.

\begin{figure}[t]
    \def\MathparLineskip{\lineskip=3pt}
    Primitive reductions:
    \vspace{-1.5ex}
    \begin{mathpar}
        \begin{bussproof}[red-app-M]
            \bussAx{
                (\lam x . M)\ N
                \aredd
                M \{ N/x \}
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-app-A]
            \bussAx{
                (\alpha x . M) \at N
                \aredd
                M \{ N/x \}
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-let-unit-M]
            \bussAx{
                \tLet \mUnit = \mUnit \tIn M
                \aredd
                M
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-let-unit-A]
            \bussAx{
                \tLet \aUnit = \aUnit \tIn M
                \aredd
                M
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-let-pair]
            \bussAx{
                \tLet \<x,y\> = \<M_1,M_2\> \tIn N
                \aredd
                N \{ M_1/x,M_2/y \}
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-proj-pair]
            \bussAssume{
                i \in \{1,2\}
            }
            \bussUn{
                \pi_i(M_1,M_2)
                \aredd
                M_i
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-case-sel]
            \bussAssume{
                i \in \{1,2\}
            }
            \bussUn{
                \tCase \tSel_i(M) \tOf \{ 1(x_1):N_1 , 2(x_2):N_2 \}
                \aredd
                N_i \{ M/x_i \}
            }
        \end{bussproof}
    \end{mathpar}

    \dashes

    Lifted reductions:
    \vspace{-1.5ex}
    \begin{mathpar}
        \begin{bussproof}[red-ctx-app-M]
            \bussAssume{
                M
                \aredd
                M'
            }
            \bussUn{
                M\ N
                \aredd
                M'\ N
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-ctx-app-A]
            \bussAssume{
                M
                \aredd
                M'
            }
            \bussUn{
                M \at N
                \aredd
                M' \at N
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-ctx-let]
            \bussAssume{
                M
                \aredd
                M'
            }
            \bussAssume{
                p \in \{\mUnit,\aUnit,\<x,y\>\}
            }
            \bussBin{
                \tLet p = M \tIn N
                \aredd
                \tLet p = M' \tIn N
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-ctx-proj]
            \bussAssume{
                M
                \aredd
                M'
            }
            \bussUn{
                \pi_i M
                \aredd
                \pi_i M'
            }
        \end{bussproof}
        \and
        \begin{bussproof}[red-ctx-case]
            \bussAssume{
                M
                \aredd
                M'
            }
            \bussUn{
                \tCase M \tOf \{ 1(x_1):N_1 , 2(x_2):N_2 \}
                \aredd
                \tCase M' \tOf \{ 1(x_1):N_1 , 2(x_2):N_2 \}
            }
        \end{bussproof}
    \end{mathpar}

    \caption{Reduction rules for the \alcalc.}
    \label{f:alphalambda:reduction}
\end{figure}

Rules~\ruleLabel{red-app-M} and~\ruleLabel{red-app-A} ($\beta$-)reduce function applications to substitutions.
Rules~\ruleLabel{red-let-unit-A} and~\ruleLabel{red-let-unit-A} eliminate unit-lets.
Rule~\ruleLabel{red-let-pair} unpacks pairs into substitutions.
Rule~\ruleLabel{red-proj-pair} projects pairs.
Rule~\ruleLabel{red-case-sel} selects a branch and substitutes accordingly.
The other rules in \Cref{f:alphalambda:reduction} close reduction under call-by-value evaluation contexts.

\fi
%</alphalambda:alphalambda:reduction>
Selected reduction rules are given in the bottom of \Cref{fig:alpha_lambda_typing}.

\paragraph{Typed translation}
\begin{figure}[t]
  \adjustfigure[\footnotesize]
  \input{figures/alcalc_translation_short}
  \caption{Translation from \alcalc to \piBI (selected clauses).}
  \label{fig:translation}
\end{figure}

%<*alphalambda:trans:trans>
Given a typed term $\Delta \vdash M : A$ and a name $z \notin \fv(M)$, we inductively translate the typing derivation of $M$ to a typing derivation for a process in \piBI, denoted $\Delta \vdash \alTrans(\Delta \vdash M : A)z \typInf z:A$.
As customary in translations of $\lambda$ into $\pi$ (cf.\ \cite{journal/mscs/Milner92,book/SangiorgiW03,journal/jfp/Wadler14}), the parameter $z$ is a name on which the behavior of the source term $M$ is made available.
By abuse of notation, we often write $\Delta \vdash \alTrans(M)z \typInf z:A$.

\begin{figure}[p]
    \small
    \def\defaultHypSeparation{\hskip1mm}
    \begin{tabular}{cc}
        Typing rule for \alcalc term $M$
        &
        \pibi translation $\alTrans(M)z$
        \\ \hline
        $\begin{bussproof}[typ-id](c)
            \bussAx{
                x:A \vdash x : A
            }
        \end{bussproof}$
        &
        $\pFwd [z<>x]$
        \\
        $\begin{bussproof}[typ-weaken](c)
            \bussAssume{
                \bunchCtx{\Gamma}[\Delta] \vdash M : A
            }
            \bussUn{
                \bunchCtx{\Gamma}[\Delta ; \Delta'] \vdash M : A
            }
        \end{bussproof}$
        &
        $\pSpw[x->\emptyset | x \in \fv(\Delta')] ; \alTrans(M)z$
        \\
        $\begin{bussproof}[typ-contract](c)
            \bussAssume{
                \bunchCtx{\Gamma}[\idx{\Delta}{1} ; \idx{\Delta}{2}] \vdash M : A
            }
            \bussUn{
                \bunchCtx{\Gamma}[\Delta] \vdash M \{ x/\idx{x}{1},x/\idx{x}{2} \mid x \in \fv(\Delta) \} : A
            }
        \end{bussproof}$
        &
        $\pSpw[x->x_1,x_2] ; \alTrans(M)z$
        \\
        $\begin{bussproof}[typ-wand-I](c)
            \bussAssume{
                \Delta , x:A \vdash M : B
            }
            \bussUn{
                \Delta \vdash \lam x . M : A \wand B
            }
        \end{bussproof}$
        &
        $\pIn z(x) ; \alTrans(M)z$
        \\
        $\begin{bussproof}[typ-wand-E](c)
            \bussAssume{
                \Delta \vdash M : A \wand B
            }
            \bussAssume{
                \Theta \vdash N : A
            }
            \bussBin{
                \Delta , \Theta \vdash M\ N : B
            }
        \end{bussproof}$
        &
        $\pRes{x} \big( \alTrans(M)x \| \pOut* x[y] ; ( \alTrans(N)y \| \pFwd [z<>x] ) \big)$
        \\
        $\begin{bussproof}[typ-emp-I](c)
            \bussAx{
                \mEmpty \vdash \mUnit : \mOne
            }
        \end{bussproof}$
        &
        $\pClose z[]$
        \\
        $\begin{bussproof}[typ-emp-E](c)
            \bussAssume{
                \Delta \vdash M : \mOne
            }
            \bussAssume{
                \bunchCtx{\Gamma}[\mEmpty] \vdash N : A
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta] \vdash \tLet \mUnit = M \tIn N : A
            }
        \end{bussproof}$
        &
        $\pRes{x} \big( \alTrans(M)x \| \pWait x() ; \alTrans(N)z \big)$
        \\
        $\begin{bussproof}[typ-sep-I](c)
            \bussAssume{
                \Delta \vdash M : A
            }
            \bussAssume{
                \Theta \vdash N : B
            }
            \bussBin{
                \Delta , \Theta \vdash \<M,N\> : A \sep B
            }
        \end{bussproof}$
        &
        $\pOut* z[y] ; \big( \alTrans(M)y \| \alTrans(N)z \big)$
        \\
        $\begin{bussproof}[typ-sep-E](c)
            \bussAssume{
                \Delta \vdash M : A \sep B
            }
            \bussAssume{
                \bunchCtx{\Gamma}[x:A , y:B] \vdash N : C
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta] \vdash \tLet \<x,y\> = M \tIn N : C
            }
        \end{bussproof}$
        &
        $\pRes{y} \big( \alTrans(M)y \| \pIn y(x) ; \alTrans(N)z \big)$
        \\
        $\begin{bussproof}[typ-conj-E](c)
            \bussAssume{
                \Delta \vdash M : A_1 \land A_2
            }
            \bussUn{
                \Delta \vdash \pi_1 M : A_1
            }
        \end{bussproof}$
        &
        $\pRes{x_2} \big( \alTrans(M){x_2} \| \pIn x_2(x_1) ; \pSpw[x_2->\emptyset] ; \pFwd [z<>x_1] \big)$
        \\
        $\begin{bussproof}[typ-conj-E](c)
            \bussAssume{
                \Delta \vdash M : A_1 \land A_2
            }
            \bussUn{
                \Delta \vdash \pi_2 M : A_2
            }
        \end{bussproof}$
        &
        $\pRes{x_2} \big( \alTrans(M){x_2} \| \pIn x_2(x_1) ; \pSpw[x_1->\emptyset] ; \pFwd [z<>x_2] \big)$
        \\
        $\begin{bussproof}[typ-disj-I](c)
            \bussAssume{
                \Delta \vdash M : A_1
            }
            \bussUn{
                \Delta \vdash \tSel_1(M) \vdash A_1 \lor A_2
            }
        \end{bussproof}$
        &
        $\pSelL z ; \alTrans(M)z$
        \\
        $\begin{bussproof}[typ-disj-I](c)
            \bussAssume{
                \Delta \vdash M : A_2
            }
            \bussUn{
                \Delta \vdash \tSel_2(M) \vdash A_1 \lor A_2
            }
        \end{bussproof}$
        &
        $\pSelR z ; \alTrans(M)z$
        \\
        $\begin{bussproof}[typ-disj-E](c)
            \bussAssume{
                \Delta \vdash M : A_1 \lor A_2
            }
            \bussAssume{
                \bunchCtx{\Gamma}[x_1:A_1] \vdash N_1 : C
            }
            \noLine
            \bussBin{
                \bunchCtx{\Gamma}[x_2:A_2]
                \vdash N_2 : C
            }
            \bussUn{
                \bunchCtx{\Gamma}[\Delta] \vdash \tCase M \tOf \{ 1(x_1):N_1 , 2(x_2):N_2 \} : C
            }
        \end{bussproof}$
        &
        $\pRes{x} \big(
            \alTrans(M)x \| \pBra* x > \left\{
                \begin{array}{@{}l@{}}
                    \inl : \alTrans(N_1)z \{ x/x_1 \} , \\
                    \inr : \alTrans(N_2)z \{ x/x_2 \}
                \end{array}
            \right\}
        \big)$
        \\
        $\begin{bussproof}[typ-cut](c)
            \bussAssume{
                \Delta \vdash M : A
            }
            \bussAssume{
                \bunchCtx{\Gamma}[x:A] \vdash N : C
            }
            \bussBin{
                \bunchCtx{\Gamma}[\Delta] \vdash N \{ M/x \} : C
            }
        \end{bussproof}$
        &
        $\pRes{x} \big( \alTrans(M)x \| \alTrans(N)z \big)$
    \end{tabular}

    \caption{Translation of \alcalc typing rules into \pibi (omitting Rule~\ruleLabel{typ-cong} and several additive rules).}
    \label{f:alphalambda:trans}
\end{figure}

The translation is inspired by a canonical translation of proofs in natural deduction into sequent calculi (cf.\ \cite[Section 6.3]{book/Pym13}), and it is type-preserving by construction.
\ifthesis
\Cref{f:alphalambda:trans} gives the translation of \alcalc typing rules.
The (derivation of) typings of the translated processes are omitted; as mentioned before, the typings are the same as for the source terms.
\ifappendix \Cref{as:alphalambda:trans} \else \cite{thesis/vdHeuvel24ex} \fi includes translations (including those omitted here) with full typing derivations.
The figure omits the translation of Rule~\ruleLabel{typ-cong}, as it translates directly to Rule~\ruleLabel{typ-cong} of \piBI.
The figure also omits the translations of several additive typing rules, because their translations are equivalent to those of their multiplicative counterparts.

\else
The translations of selected rules from \cref{fig:alpha_lambda_typing} is given in \cref{fig:translation}.
\fi
The identity derivation is translated into a forwarder.
Introduction rules are translated using right rules for the associated connectives, and elimination rules are translated using the corresponding left rule in combination with a cut.
Weakening and contraction, which use implicit substitutions in the \alcalc, are translated using the explicit spawn construct.

The following example features the translation of an interesting term, including the full typing derivation of the translated process.

\begin{figure}[t]
    \[
        \def\defaultHypSeparation{\hskip.3ex}
        \def\ScoreOverhang{1pt}
        \begin{bussproof}
            \bussAx{
                \begin{array}[t]{@{}l@{}}
                    y:A \to A \to B
                    \\
                    \vdash \alTrans(y)w = \pFwd [w<>y]
                    \\
                    \typInf w:A \to A \to B
                \end{array}
            }
            \bussAx{
                \begin{array}[t]{@{}l@{}}
                    a_2:A
                    \\
                    \vdash \alTrans(a_2){a'_2} = \pFwd [a'_2<>a_2]
                    \\
                    \typInf a'_2:A
                \end{array}
            }
            \bussAx{
                \begin{array}[t]{@{}l@{}}
                    w:A \to B
                    \\
                    \vdash \pFwd [x<>w]
                    \\
                    \typInf x:A \to B
                \end{array}
            }
            \bussBin{
                \begin{array}[t]{@{}l@{}}
                    a_2:A ; w:A \to A \to B
                    \\
                    \vdash \pOut* w[a'_2] ; ( \alTrans(a_2){a'_2} \| \pFwd[x<>w] )
                    \\ \typInf x:A \to B
                \end{array}
            }
            \bussBin{
                \begin{array}[t]{@{}l@{}}
                    a_2:A ; y:A \to A \to B
                    \\
                    \vdash \alTrans(M_4)x = \pRes{w} \big( \alTrans(y)w \| \pOut* w[a'_2] ; ( \alTrans(a_2){a'_2} \| \pFwd[x<>w] ) \big)
                    \\
                    \typInf x:A \to B
                \end{array}
            }
            \bussAx{
                \begin{array}[t]{@{}l@{}}
                    a_1:A
                    \\
                    \vdash \alTrans(a_1){a'_1} = \pFwd [a'_1<>a_1]
                    \\
                    \typInf a'_1:A
                \end{array}
            }
            \bussAx{
                \begin{array}[t]{@{}l@{}}
                    x:B
                    \\
                    \vdash \pFwd [z<>x]
                    \\
                    \typInf z:B
                \end{array}
            }
            \bussBin{
                \begin{array}[t]{@{}l@{}}
                    a_1:A ; x:A \to B
                    \\
                    \vdash \pOut* x[a'_1] ; ( \alTrans(a_1){a'_1} \| \pFwd [z<>x] )
                    \\
                    \typInf z:B
                \end{array}
            }
            \bussBin{
                a_1:A ; a_2:A ; y:A \to A \to B \vdash \alTrans(M_3)z = \pRes{x} \big( \alTrans(M_4)x \| \pOut* x[a'_1] ; ( \alTrans(a_1){a'_1} \| \pFwd [z<>x] ) \big) \typInf z:B
            }
            \bussUn{
                    a:A ; y:A \to A \to B \vdash \alTrans(M_2)z = \pSpw[a->a_1,a_2] ; \alTrans(M_3)z \typInf z:B
            }
            \bussUn{
                a:A \vdash \alTrans(M_1)z = \pIn z(y) ; \alTrans(M_2)z \typInf z:(A \to A \to B) \to B
            }
            \bussUn{
                \mEmpty \vdash \alTrans(M)z = \pIn z(a) ; \alTrans(M_1)z \typInf z:A \wand (A \to A \to B) \to B
            }
        \end{bussproof}
    \]
    
    \caption{Typing derivation of an \alcalc term into \pibi (cf.\ \Cref{x:alphalambda:trans}).}\label{f:alphalambda:x:trans}
\end{figure}

\begin{example}
    \label{x:alphalambda:trans}
    Consider the following \alcalc derivation of $M \deq \lam a . \alpha y . (y \at a) \at a$:
    \[
        \begin{bussproof}
            \bussAx{
                a_2:A \vdash a_2 : A
            }
            \bussAx{
                y:A \to A \to B \vdash y : A \to A \to B
            }
            \bussBin{
                a_2:A ; y:A \to A \to B \vdash M_4 \deq y \at a_2 : A \to B
            }
            \bussAx{
                a_1:A \vdash a_1 : A
            }
            \bussBin{
                a_1:A ; a_2:A ; y:A \to A \to B \vdash M_3 \deq (y \at a_2) \at a_1 : B
            }
            \bussUn{
                a:A ; y:A \to A \to B \vdash M_2 \deq (y \at a) \at a : B
            }
            \bussUn{
                a:A \vdash M_1 \deq \alpha y . (y \at a) \at a : (A \to A \to B) \to B
            }
            \bussUn{
                \mEmpty \vdash M = \lam a . \alpha y . (y \at a) \at a : A \wand (A \to A \to B) \to B
            }
        \end{bussproof}
    \]
    The translation of $M$ into \piBI is
    \[
        \alTrans(M)z = \pIn z(a) ; \pIn z(y) ; \pSpw[a->a_1,a_2] ; \pRes{x} \begin{array}[t]{@{}l@{}}
            \big( \pRes{w} ( \pFwd [w<>y] \| \pOut* w[a'_2] ; ( \pFwd [a'_2<>a_2] \| \pFwd[x<>w] ) )
            \\
            {} \| \pOut* x[a'_1] ; ( \pFwd [a'_1<>a_1] \| \pFwd [z<>x] ) \big)
        \end{array}
    \]
    \Cref{f:alphalambda:x:trans} gives the typing of $\alTrans(M)z$ in \piBI.
    \ifthesis\else
    This corresponds to the \piBI derivation in \cref{ex:unusual}, modulo additional cuts on forwarders due to the translation of variables and function applications.
    \fi
\end{example}
%</alphalambda:trans:trans>

\subsection{Operational Correspondence}

%<*alphalambda:trans:oc>
Here we show that the translation $\alTrans(-)z$ preserves and reflects behavior of terms and processes.
We formulate this important property in terms of an \emph{operational correspondence} result, following established criteria (cf.\ \cite{conf/express/Peters19,journal/ic/Gorla10}).
Concretely, we establish the result in two parts: \emph{completeness} and \emph{soundness}.
The former states that reduction of \alcalc terms induces corresponding reductions of their process translations into \piBI.
The latter states that reductions of translated terms are reflected by corresponding reductions of source terms in the \alcalc.
\ifappendix \Cref{as:alphalambda:trans} \else \cite{thesis/vdHeuvel24ex} \fi gives detailed proofs.
%</alphalambda:trans:oc>

\subsubsection{Completeness}

%<*alphalambda:trans:oc:completeness>
For completeness, we want to mimic every \alcalc reduction with one or multiple \piBI reductions.
That is, we would like to show that the translation induces a simulation.
To accurately characterize this, we need to address the discrepancy between the way substitutions and function applications are handled in \alcalc and \piBI.

Unfortunately, the reductions of a translated \piBI process might diverge from the source term, due to the way substitutions and function applications are handled in the \alcalc.
A function application $(\alpha x . M) \at N$ results in a term with a substitution $M \{ N/x \}$.
If there are multiple occurrences of $x$ in $M$---which is possible due to contraction---, they all get substituted with $N$.
On the \piBI side, substitution is represented as a composition \mbox{$\pRes{x} \big( \alTrans(N)x \| \alTrans(M)z \big)$}, in which \emph{one copy} of $\alTrans(N)x$ gets connected with the body $\alTrans(M)z$ through the endpoint~$x$.
The contraction of the multiple occurrences of $x$ in $M$ is handled with a spawn prefix in~$\alTrans(M)z$.

To address this discrepancy, we formulate completeness in a generalized way: following the approach by Toninho \etal~\cite{conf/fossacs/ToninhoCP12}, we define a \emph{substitution lifting} relation which we show to be a simulation.

\begin{definition}[Substitution Lifting]
    \label{d:alphalambda:substLift}
    Given a term $M$ and a process $P$ of the same typing, we say $P$ lifts the substitutions of $M$, denoted $\Delta \vdash P \subLift M \typInf z:A$, or $P \subLift M$ for short, if:
    \begin{enumerate}
        \item
            $P \equiv \pSpw[\spvar_s] ; \ldots ; \pSpw[\spvar_1] ; \pRes{x_n} \big( \alTrans(N_n){x_n} \| \ldots \pRes{x_1} ( \alTrans(N_1){x_1} \| \alTrans(M')z ) \ldots \big)$ where for each $i \in [1,s]$, $\spvar_i = \map{y_1->\emptyset;\ldots;y_m->\emptyset}$ or $\spvar_i = \map{y_1->\idx{y_1}{1},\idx{y_1}{2};\ldots;y_m->\idx{y_m}{1},\idx{y_m}{2}}$;

        \item
            $M = M' \{ N_1/x_1,\ldots,N_n/x_n \} \{ \tilde{\spvar_1},\ldots,\tilde{\spvar_s} \}$ where for each $i \in [1,s]$, $\tilde{\spvar_i}$ denotes a substitution corresponding to the binding $\spvar_i$.
            Specifically, $\tilde{\spvar_i}$ is an empty substitution if $\spvar_i$ is weakening,
            and is the substitution $\{ y_1/\idx{y_1}{1},y_1/\idx{y_1}{2},\ldots,y_m/\idx{y_m}{1},y_m/\idx{y_m}{2} \}$ if $\spvar_i$ is contraction.
    \end{enumerate}
    That is, both $P$ and $M$ are composed of $n$ cuts with (the translations of) the terms $M,N_1,\ldots,N_n$.
\end{definition}

\noindent
Note that for any well-typed $N$ we have $\alTrans(N)z \subLift N$.

We now show the completeness result.

\begin{restatable}[Completeness]{theorem}{tAlphalambdaCompleteness}
    \label{t:alphalambda:completeness}
    Suppose given $\Delta \vdash M : A$ and $\Delta \vdash P \typInf z:A$ such that $P \subLift M$.
    If $M \aredd N$, then there exists $Q$ such that $P \redd* Q \subLift N$.
\end{restatable}

\begin{sketch}
    We first prove separately a basic version of completeness without substitution lifting; this follows by induction on the derivation of the term reduction.
    Then, we distinguish cases on the source of the reduction: from a substitution, or from the term itself.
    In the former case, we can argue that the forwarder representing the subsitution is not blocked; hence, the substitution can be resolved and the reduction mimicked following basic completeness.
    The latter case follows from basic completeness directly.
\end{sketch}
%</alphalambda:trans:oc:completeness>

% \begin{proof}
%   Since $P \subLift M$, we can write the latter as $M'\subst{x_1->N_1,,x_n->N_n}$.
%   We then consider two cases, depending on whether the reduction $M \aredd N$ already happens in $M'$, or whether this reduction is triggered by one of the substitutions.

%   In the first case we already have a reduction $M' \aredd N'$ that is ``lifted'' to the reduction $$M = M'\subst{x_1->N_1,,x_n->N_n} \aredd N'\subst{x_1->N_1,,x_n->N_n} = N.$$
%   We can the directly appeal to \Cref{lem:basic_completeness}.

%   In the second case, the reduction in the term is only some substitution $\subst{x_i->N_i}$ is performed.
%   The idea is to reduce this to the first case, by explicitly performing the substitution $\subst{x_i->N_i}$ in the corresponding processes.

%   If $\subst{x_i->N_i}$ is the substitution that enables the reduction $M'\subst{x_1->N_1,,x_n->N_n} \aredd N$, then the variable $x_i$ is located at a head position in the term $M'$.
%   That is, under the translation, the sub-process $\bTrans_y(x_i) = \fwd[y <- x_i]$ will not occur in $\bTrans_z(M)$ under an input/output prefix, which will allow us to eagerly perform the substitution by using the forwarder reduction and spawn propagation reductions, if needed.
% \end{proof}

\subsubsection{Soundness}

%<*alphalambda:trans:oc:soundness>
Completeness (\Cref{t:alphalambda:completeness}) shows that the reductions of terms are preserved by the translation.
We now show that reductions of translated processes are reflected by reductions of source terms.
However, there is a caveat: the translated processes are ``more concurrent'', and have more possible reductions that cannot be immediately matched in source terms.

\begin{example}
    For some term $M \{ N/x \}$ and a corresponding substitution-lifted process $P \deq \pRes{x} \big( \alTrans(N)x \| \alTrans(M)z \big)$,
    suppose that the subterm $N$ has a reduction $N \aredd N'$.
    The process $P$ can mimic this reduction:
    \[
        P \redd \pRes{x} \big( Q \| \alTrans(M)z \big),
    \]
    for some $Q$.
    However, we do not necessarily have a corresponding \mbox{$M \{ N/x \} \aredd M \{ N'/x \}$}, since the variable $x$ might occur at a position where it is not enabled (e.g., under a $\lam$-binder).
\end{example}

In order to be able to reflect all the reductions in translated processes, we state soundness in terms of an extended class of reductions for terms, denoted $\afredd$ (with reflexive, transitive closure denoted $\afredd*$).
To be precise, let $\evalCtx{C}$ be an arbitrary \alcalc context.
In addition to the reductions in \Cref{f:alphalambda:reduction}, we consider reductions under arbitrary contexts:
\[
    \begin{bussproof}[red-arbitrary-ctx]
        \bussAssume{
            M \afredd N
        }
        \bussUn{
            \evalCtx{C}[M] \afredd \evalCtx{C}[N]
        }
    \end{bussproof}
\]

\begin{restatable}[Soundness]{theorem}{tAlphalambdaSoundness}
    \label{t:alphalambda:soundness}
    Given $\Delta \vdash P \subLift M \typInf z:A$, if $P \redd* Q$, then there exist $N$ and $R$ such that $M \afredd* N$ and $Q \redd* R \subLift N$.
\end{restatable}

\begin{sketch}
    By cases on the possible reductions of $P$, informed by the structure and typing of the source term $M$.
    The key point in the proof is to postpone certain independent reductions of the target process, which cannot be immediately matched by reductions in the source term.
\end{sketch}

Note that the premise in \Cref{t:alphalambda:soundness} permits arbitrarily many reduction steps from $P$ to $Q$ (i.e., $P \redd* Q$), assuring that \emph{every} sequence of reductions of $P$ is reflected by a corresponding sequence of reductions of the source term $M$.
The alternative, with a single reduction in the premise (i.e., $P \redd Q$), is a much weaker property.
%</alphalambda:trans:oc:soundness>

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

